Bypassing LLM Watermarks with Color-Aware Substitutions

Watermarking approaches are proposed to identify if text being circulated is human or large language model (LLM) generated. The state-of-the-art watermarking strategy of Kirchenbauer et al. (2023a) biases the LLM to generate specific (``green'') tokens. However, determining the robustness of this watermarking method is an open problem. Existing attack methods fail to evade detection for longer text segments. We overcome this limitation, and propose {\em Self Color Testing-based Substitution (SCTS)}, the first ``color-aware'' attack. SCTS obtains color information by strategically prompting the watermarked LLM and comparing output tokens frequencies. It uses this information to determine token colors, and substitutes green tokens with non-green ones. In our experiments, SCTS successfully evades watermark detection using fewer number of edits than related work. Additionally, we show both theoretically and empirically that SCTS can remove the watermark for arbitrarily long watermarked text.

==> contents/6_2_old_tables.tex <==
\begin{table*}[!t]
\centering
\caption{AUROC table comparing different methods. The columns 0, 0.05,..., 0.5, 1 represent budgets.}
\label{tab:my_label}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} & RP1 & \multirow{8}{*}{0.9984} &  & 0.9964 &  & 0.9964 &  & 0.9964 &  & 0.992 &  & 0.994 & 0.7994 \\
& RP2 &  &  & 0.9964 &  & 0.9964 &  & 0.9964 &  & 0.992 &  & 0.9908 & 0.9252 \\
& RP3 &  &  & 0.9964 &  & 0.9964 &  & 0.9972 &  & 0.9912 &  & 0.9928 & 0.775 \\
& RP4 &  &  & 0.9964 &  & 0.9964 &  & 0.9972 &  & 0.9904 &  & 0.9892 & 0.8176 \\
& RP5 &  &  & 0.9964 &  & 0.9964 &  & 0.9972 &  & 0.9904 &  & 0.9912 & \textbf{0.7248} \\
& SICO &  &  & 0.996 &  & 0.996 &  & 0.996 &  & 0.996 &  & 0.9892 & 0.8716 \\
& RB &  & 0.9892 & 0.9816 & 0.9732 & 0.96 & 0.9524 & 0.932 & 0.9024 & 0.8744 & 0.8134 & 0.7488 & \\
& \textbf{SCTS} &  & \textbf{0.9812} & \textbf{0.952} & \textbf{0.9048} & \textbf{0.8152} & \textbf{0.6984} & \textbf{0.5272} & \textbf{0.3168} & \textbf{0.2932} & \textbf{0.2932} & \textbf{0.2932} & \textbf{} \\
\midrule
% c = 2
\multirow{8}{*}{2} & RP1 & \multirow{8}{*}{0.9948} &  & 0.9924 &  & 0.9924 &  & 0.9924 &  & 0.9915 &  & 0.9627 & 0.8313 \\
& RP2 &  &  & 0.9924 &  & 0.9924 &  & 0.9924 &  & 0.9915 &  & 0.9641 & 0.8582 \\
& RP3 &  &  & 0.9924 &  & 0.9924 &  & 0.9924 &  & 0.9910 &  & 0.9669 & 0.6432 \\
& RP4 &  &  & 0.9924 &  & 0.9924 &  & 0.9924 &  & 0.9910 &  & 0.9646 & 0.7179 \\
& RP5 &  &  & 0.9924 &  & 0.9924 &  & 0.9924 &  & 0.9915 &  & 0.9612 & \textbf{0.6186} \\
& SICO &  &  & 0.9929 &  & 0.9929 &  & 0.99197 &  & 0.9929 &  & 0.9731 & 0.7817 \\
& RB &  & 0.9887 & 0.9773 & 0.9617 & 0.9598 & 0.9523 & 0.9315 & 0.8885 & 0.8273 & 0.7226 & 0.6782 & \\
& \textbf{SCTS} &  & \textbf{0.9825} & \textbf{0.9575} & \textbf{0.9012} & \textbf{0.8181} & \textbf{0.6356} & \textbf{0.409} & \textbf{0.2424} & \textbf{0.2018} & \textbf{0.2018} & \textbf{0.2018} & \textbf{} \\
\midrule
% c = 3
\multirow{8}{*}{3} & RP1 & \multirow{8}{*}{0.9952} &  & 0.9878 &  & 0.9878 &  & 0.9878 &  & 0.9648 &  & 0.9818 & 0.8587 \\
& RP2 &  &  & 0.9878 &  & 0.9878 &  & 0.9878 &  & 0.9627 &  & 0.9822 & 0.8377 \\
& RP3 &  &  & 0.9878 &  & 0.9878 &  & 0.9813 &  & 0.9618 &  & 0.9800 & 0.7229 \\
& RP4 &  &  & 0.9878 &  & 0.9878 &  & 0.9865 &  & 0.9618 &  & 0.9787 & 0.7463 \\
& RP5 &  &  & 0.9878 &  & 0.9878 &  & 0.9865 &  & 0.9557 &  & 0.9844 & \textbf{0.6415} \\
& SICO &  &  & 0.9896 &  & 0.9896 &  & 0.9874 &  & 0.9896 &  & 0.9709 & 0.8867 \\
& RB &  & 0.9753 & 0.9644 & 0.9581 & 0.9227 & 0.9138 & 0.875 & 0.8277 & 0.7526 & 0.6278 & 0.6278 & \\
& \textbf{SCTS} &  & \textbf{0.9694} & \textbf{0.9271} & \textbf{0.8628} & \textbf{0.7513} & \textbf{0.5352} & \textbf{0.3058} & \textbf{0.1411} & \textbf{0.1289} & \textbf{0.1289} & \textbf{0.1289} & \textbf{} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


\begin{table*}[!t]
\centering
\caption{SuccessRate comparison between RB, SCTS, and other methods across different budgets.}
\label{tab:success_rate}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} & RP1 & \multirow{8}{*}{0.8200} &  & 0.7200 &  & 0.7200 &  & 0.7200 &  & 0.7000 &  & 0.6600 & 0.0400 \\
& RP2 &  &  & 0.7200 &  & 0.7000 &  & 0.7000 &  & 0.7000 &  & 0.5400 & 0.1600 \\
& RP3 &  &  & 0.7200 &  & 0.7000 &  & 0.6600 &  & 0.5800 &  & 0.5000 & 0.0200 \\
& RP4 &  &  & 0.7200 &  & 0.6800 &  & 0.6600 &  & 0.5400 &  & 0.4200 & 0.0200 \\
& RP5 &  &  & 0.7200 &  & 0.6800 &  & 0.6600 &  & 0.5400 &  & 0.4200 & 0.0000 \\
& SICO &  &  & 0.7200 &  & 0.7000 &  & 0.6800 &  & 0.7000 &  & 0.6000 & 0.1800 \\
& RB &  & 0.5600 & 0.4000 & 0.2800 & 0.1800 & 0.1000 & 0.0800 & 0.0600 & 0.0000 & 0.0000 & 0.0000 &  \\
& SCTS &  & 0.4600 & 0.2200 & 0.1000 & 0.0200 & 0.0200 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 &  \\
\midrule
% c = 2
\multirow{8}{*}{2} & RP1 & \multirow{8}{*}{0.8478} &  & 0.8043 &  & 0.8043 &  & 0.8043 &  & 0.8043 &  & 0.6522 & 0.0217 \\
& RP2 &  &  & 0.8043 &  & 0.7609 &  & 0.7174 &  & 0.6304 &  & 0.1304 & 0.1304 \\
& RP3 &  &  & 0.8043 &  & 0.7391 &  & 0.6522 &  & 0.4783 &  & 0.0000 & 0.0000 \\
& RP4 &  &  & 0.8043 &  & 0.7174 &  & 0.6087 &  & 0.3913 &  & 0.0435 & 0.0435 \\
& RP5 &  &  & 0.8043 &  & 0.7174 &  & 0.5870 &  & 0.3478 &  & 0.0000 & 0.0000 \\
& SICO &  &  & 0.8043 &  & 0.7826 &  & 0.7174 &  & 0.7826 &  & 0.5435 & 0.2391 \\
& RB &  & 0.7391 & 0.5652 & 0.3696 & 0.3043 & 0.1087 & 0.0652 & 0.0217 & 0.0000 & 0.0000 & 0.0000 &  \\
& SCTS &  & 0.6087 & 0.2826 & 0.0870 & 0.0435 & 0.0217 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 &  \\
\midrule
% c = 3
\multirow{8}{*}{3} & RP1 & \multirow{8}{*}{0.7917} &  & 0.7500 &  & 0.7500 &  & 0.7500 &  & 0.7083 &  & 0.6250 & 0.0417 \\
& RP2 &  &  & 0.7292 &  & 0.7083 &  & 0.6250 &  & 0.5833 &  & 0.1458 & 0.1458 \\
& RP3 &  &  & 0.7292 &  & 0.6667 &  & 0.6250 &  & 0.4583 &  & 0.0208 & 0.0208 \\
& RP4 &  &  & 0.7292 &  & 0.6667 &  & 0.6042 &  & 0.3958 &  & 0.0417 & 0.0417 \\
& RP5 &  &  & 0.7292 &  & 0.6458 &  & 0.6042 &  & 0.3333 &  & 0.0208 & 0.0208 \\
& SICO &  &  & 0.7708 &  & 0.7708 &  & 0.7500 &  & 0.7500 &  & 0.6042 & 0.1875 \\
& RB &  & 0.6250 & 0.4167 & 0.3125 & 0.2083 & 0.0833 & 0.0208 & 0.0000 & 0.0000 & 0.0000 & 0.0000 &  \\
& SCTS &  & 0.5417 & 0.2500 & 0.0833 & 0.0208 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Time in Seconds comparison between RP, SICO, RB, and SCTS methods across different budgets.}
\label{tab:time_seconds}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} 
& RP1 & \multirow{8}{*}{0.0} &  & 185.7 &  & 182.0 &  & 181.7 &  & 180.9 &  & 188.3 & 186.2 \\
& RP2 &  &  & 369.7 &  & 366.8 &  & 360.5 &  & 360.0 &  & 377.1 & 372.3 \\
& RP3 &  &  & 565.6 &  & 556.1 &  & 542.8 &  & 546.4 &  & 560.0 & 492.5 \\
& RP4 &  &  & 740.9 &  & 736.7 &  & 732.5 &  & 716.3 &  & 720.1 & 588.7 \\
& RP5 &  &  & 925.8 &  & 917.8 &  & 912.8 &  & 879.5 &  & 862.7 & 661.8 \\
& SICO &  &  & 1238.9 &  & 1837.5 &  & 2501.9 &  & 3259.4 &  & 2500.6 & 3003.1 \\
& RB &  & 24.6 & 49.8 & 74.6 & 99.6 & 123.9 & 148.2 & 172.3 & 196.5 & 219.9 & 243.9 &  \\
& SCTS &  & 7370.2 & 15242.5 & 23398.6 & 31427.0 & 39054.6 & 46890.8 & 54810.6 & 59475.0 & 59625.7 & 59625.7 &  \\
\midrule
% c = 2
\multirow{8}{*}{2} 
& RP1 & \multirow{8}{*}{0.0} &  & 131.4 &  & 132.1 &  & 133.0 &  & 129.5 &  & 137.0 & 132.0 \\
& RP2 &  &  & 238.5 &  & 235.5 &  & 232.1 &  & 229.2 &  & 242.7 & 247.6 \\
& RP3 &  &  & 343.3 &  & 337.0 &  & 330.7 &  & 324.5 &  & 335.7 & 335.1 \\
& RP4 &  &  & 447.2 &  & 441.3 &  & 425.9 &  & 425.2 &  & 424.0 & 406.8 \\
& RP5 &  &  & 548.0 &  & 551.8 &  & 517.6 &  & 517.3 &  & 502.6 & 464.7 \\
& SICO &  &  & 1066.3 &  & 1767.7 &  & 2466.8 &  & 3230.1 &  & 2457.2 & 3007.3 \\
& RB &  & 12.3 & 25.0 & 37.4 & 49.8 & 62.0 & 74.0 & 85.9 & 97.96 & 109.6 & 122.0 &  \\
& SCTS &  & 5330.0 & 11178.2 & 16757.3 & 22290.3 & 27931.1 & 33361.3 & 38560.4 & 41418.0 & 41513.4 & 41513.4 &  \\
\midrule
% c = 3
\multirow{8}{*}{3} 
& RP1 & \multirow{8}{*}{0.0} &  & 140.6 &  & 135.4 &  & 134.0 &  & 136.2 &  & 133.2 & 137.4 \\
& RP2 &  &  & 250.1 &  & 256.1 &  & 252.0 &  & 242.6 &  & 236.4 & 261.7 \\
& RP3 &  &  & 353.6 &  & 373.1 &  & 358.8 &  & 342.5 &  & 342.7 & 365.8 \\
& RP4 &  &  & 459.8 &  & 503.9 &  & 454.0 &  & 431.3 &  & 452.8 & 455.6 \\
& RP5 &  &  & 562.7 &  & 624.1 &  & 557.9 &  & 517.0 &  & 553.0 & 531.1 \\
& SICO &  &  & 1110.5 &  & 1755.2 &  & 2476.0 &  & 3317.1 &  & 2461.6 & 2987.2 \\
& RB &  & 12.7 & 25.7 & 38.6 & 51.2 & 63.8 & 76.3 & 88.5 & 100.6 & 112.3 & 44449.8 &  \\
& SCTS &  & 5435.1 & 11631.1 & 17608.0 & 23616.1 & 29753.0 & 35904.0 & 41578.9 & 44215.6 & 44324.5 & 44324.5 &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Average Time per Sample (in Seconds) comparison between RP, SCTS, RB, and SICO methods across different budgets.}
\label{tab:avg_time_per_sample}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} 
& RP1 & \multirow{8}{*}{0.0} &  & 3.71 &  & 3.64 &  & 3.63 &  & 3.62 &  & 3.77 & 3.72 \\
& RP2 &  &  & 7.39 &  & 7.34 &  & 7.21 &  & 7.20 &  & 7.54 & 7.45 \\
& RP3 &  &  & 11.31 &  & 11.12 &  & 10.86 &  & 10.93 &  & 11.20 & 9.85 \\
& RP4 &  &  & 14.82 &  & 14.73 &  & 14.65 &  & 14.33 &  & 14.40 & 11.77 \\
& RP5 &  &  & 18.52 &  & 18.36 &  & 18.26 &  & 17.59 &  & 17.25 & 13.24 \\
& SICO &  &  & 24.78 &  & 36.75 &  & 50.04 &  & 65.19 &  & 50.01 & 60.06 \\
& RB &  & 0.49 & 0.996 & 1.49 & 1.99 & 2.48 & 2.96 & 3.45 & 3.93 & 4.40 & 4.88 &  \\
& SCTS &  & 147.40 & 304.85 & 467.97 & 628.54 & 781.09 & 937.82 & 1096.21 & 1189.50 & 1192.51 & 1192.51 &  \\
\midrule
% c = 2
\multirow{8}{*}{2} 
& RP1 & \multirow{8}{*}{0.0} &  & 2.86 &  & 2.87 &  & 2.89 &  & 2.82 &  & 2.98 & 2.87 \\
& RP2 &  &  & 5.18 &  & 5.12 &  & 5.05 &  & 4.98 &  & 5.28 & 5.38 \\
& RP3 &  &  & 7.46 &  & 7.33 &  & 7.19 &  & 7.06 &  & 7.30 & 7.28 \\
& RP4 &  &  & 9.72 &  & 9.59 &  & 9.26 &  & 9.25 &  & 9.22 & 8.84 \\
& RP5 &  &  & 11.91 &  & 11.99 &  & 11.25 &  & 11.24 &  & 10.93 & 10.10 \\
& SICO &  &  & 23.19 &  & 38.42 &  & 53.63 &  & 70.22 &  & 53.42 & 65.38 \\
& RB &  & 0.27 & 0.54 & 0.81 & 1.08 & 1.35 & 1.61 & 1.87 & 2.13 & 2.38 & 2.65 &  \\
& SCTS &  & 115.87 & 243.00 & 364.29 & 484.57 & 607.20 & 726.33 & 838.27 & 900.39 & 903.33 & 903.33 &  \\
\midrule
% c = 3
\multirow{8}{*}{3} 
& RP1 & \multirow{8}{*}{0.0} &  & 2.93 &  & 2.82 &  & 2.79 &  & 2.84 &  & 2.78 & 2.86 \\
& RP2 &  &  & 5.21 &  & 5.34 &  & 5.25 &  & 5.05 &  & 4.92 & 5.45 \\
& RP3 &  &  & 7.37 &  & 7.77 &  & 7.48 &  & 7.14 &  & 7.14 & 7.62 \\
& RP4 &  &  & 9.58 &  & 10.50 &  & 9.46 &  & 8.99 &  & 9.43 & 9.49 \\
& RP5 &  &  & 11.73 &  & 13.00 &  & 11.62 &  & 10.77 &  & 11.52 & 11.06 \\
& SICO &  &  & 23.14 &  & 36.57 &  & 51.58 &  & 69.11 &  & 51.28 & 62.23 \\
& RB &  & 0.26 & 0.54 & 0.80 & 1.07 & 1.33 & 1.59 & 1.84 & 2.10 & 2.34 & 926.04 &  \\
& SCTS &  & 113.23 & 242.31 & 367.08 & 492.00 & 619.85 & 747.58 & 866.23 & 921.16 & 923.43 & 923.43 &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}



\begin{table*}[!t]
\centering
\caption{Number of LLM Calls comparison between RP, SCTS, RB, and SICO methods across different budgets.}
\label{tab:llm_calls}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} 
& RP1 & \multirow{8}{*}{0} &  & 50 &  & 50 &  & 50 &  & 50 &  & 50 & 50 \\
& RP2 &  &  & 100 &  & 100 &  & 100 &  & 100 &  & 100 & 100 \\
& RP3 &  &  & 150 &  & 150 &  & 150 &  & 150 &  & 150 & 150 \\
& RP4 &  &  & 200 &  & 200 &  & 200 &  & 200 &  & 200 & 200 \\
& RP5 &  &  & 250 &  & 250 &  & 250 &  & 250 &  & 250 & 250 \\
& SICO &  &  & 263 &  & 299 &  & 428 &  & 544 &  & 438 & 538 \\
& RB &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &  \\
& SCTS &  & 1264 & 2571 & 3853 & 5078 & 6335 & 7604 & 8351 & 8376 & 8376 & 8376 &  \\
\midrule
% c = 2
\multirow{8}{*}{2} 
& RP1 & \multirow{8}{*}{0} &  & 46 &  & 46 &  & 46 &  & 46 &  & 46 & 46 \\
& RP2 &  &  & 92 &  & 92 &  & 92 &  & 92 &  & 92 & 92 \\
& RP3 &  &  & 138 &  & 138 &  & 138 &  & 138 &  & 138 & 138 \\
& RP4 &  &  & 184 &  & 184 &  & 184 &  & 184 &  & 184 & 184 \\
& RP5 &  &  & 230 &  & 230 &  & 230 &  & 230 &  & 230 & 230 \\
& SICO &  &  & 259 &  & 295 &  & 424 &  & 540 &  & 434 & 534 \\
& RB &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &  \\
& SCTS &  & 934 & 1825 & 2703 & 3606 & 4481 & 5306 & 5759 & 5774 & 5774 & 5774 &  \\
\midrule
% c = 3
\multirow{8}{*}{3} 
& RP1 & \multirow{8}{*}{0} &  & 48 &  & 48 &  & 48 &  & 48 &  & 48 & 48 \\
& RP2 &  &  & 96 &  & 96 &  & 96 &  & 96 &  & 96 & 96 \\
& RP3 &  &  & 144 &  & 144 &  & 144 &  & 144 &  & 144 & 144 \\
& RP4 &  &  & 192 &  & 192 &  & 192 &  & 192 &  & 192 & 192 \\
& RP5 &  &  & 240 &  & 240 &  & 240 &  & 240 &  & 240 & 240 \\
& SICO &  &  & 261 &  & 297 &  & 426 &  & 542 &  & 436 & 536 \\
& RB &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &  \\
& SCTS &  & 976 & 1927 & 2891 & 3892 & 4874 & 5787 & 6210 & 6227 & 6227 & 6227 &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Number of LLM Calls per Sample comparison between RP, SCTS, RB, and SICO methods across different budgets.}
\label{tab:llm_calls_per_sample}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{8}{*}{1} 
& RP1 & \multirow{8}{*}{0.00} &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 & 1.00 \\
& RP2 &  &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 & 2.00 \\
& RP3 &  &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 & 3.00 \\
& RP4 &  &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 & 4.00 \\
& RP5 &  &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 & 5.00 \\
& SICO &  &  & 5.26 &  & 5.98 &  & 8.56 &  & 10.88 &  & 8.76 & 10.76 \\
& RB &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  \\
& SCTS &  & 25.28 & 51.42 & 77.06 & 101.56 & 126.70 & 152.08 & 167.02 & 167.52 & 167.52 & 167.52 &  \\
\midrule
% c = 2
\multirow{8}{*}{2} 
& RP1 & \multirow{8}{*}{0.00} &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 & 1.00 \\
& RP2 &  &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 & 2.00 \\
& RP3 &  &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 & 3.00 \\
& RP4 &  &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 & 4.00 \\
& RP5 &  &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 & 5.00 \\
& SICO &  &  & 5.63 &  & 6.41 &  & 9.22 &  & 11.74 &  & 9.43 & 11.61 \\
& RB &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  \\
& SCTS &  & 20.30 & 39.67 & 58.76 & 78.39 & 97.41 & 115.35 & 125.20 & 125.52 & 125.52 & 125.52 &  \\
\midrule
% c = 3
\multirow{8}{*}{3} 
& RP1 & \multirow{8}{*}{0.00} &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 &  & 1.00 & 1.00 \\
& RP2 &  &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 &  & 2.00 & 2.00 \\
& RP3 &  &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 &  & 3.00 & 3.00 \\
& RP4 &  &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 &  & 4.00 & 4.00 \\
& RP5 &  &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 &  & 5.00 & 5.00 \\
& SICO &  &  & 5.44 &  & 6.19 &  & 8.88 &  & 11.29 &  & 9.08 & 11.17 \\
& RB &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  \\
& SCTS &  & 20.33 & 40.14 & 60.23 & 81.08 & 101.54 & 120.56 & 129.38 & 129.73 & 129.73 & 129.73 &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[!t]
\centering
\caption{AUROC table comparing different methods with budgets for selfhash.}
\label{tab:reordered_comparison}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ \midrule
% c = 1
\multirow{9}{*}{1} 
& RP1 & \multirow{9}{*}{1.0} & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 \\
& RP2 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 \\
& RP3 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.99 & 0.88 \\
& RP4 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.99 & 0.86 \\
& RP5 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.99 & 0.83 \\
& SICO &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.98 & 0.93 \\
& RB &  & 1.0 & 1.0 & 1.0 & 0.98 & 0.98 & 0.98 & 0.95 & 0.94 & 0.94 & 0.94 & 0.92 \\
& SCTS &  & 0.99 & 0.98 & 0.97 & 0.97 & 0.94 & 0.9 & 0.87 & 0.84 & 0.78 & 0.66 & \\
& Oracle &  & 0.98 & 0.87 & 0.65 & 0.25 & 0.1 & 0.02 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 3
\multirow{9}{*}{3} 
& RP1 & \multirow{9}{*}{1.0} & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP2 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP3 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.98 \\
& RP4 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.74 \\
& RP5 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.76 \\
& SICO &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.98 \\
& RB &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 & \\
& SCTS &  & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.92 & 0.7 & 0.64 & 0.64 & 0.64 & \\
& Oracle &  & 1.0 & 1.0 & 1.0 & 0.88 & 0.5 & 0.12 & 0.03 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 4
\multirow{9}{*}{4} 
& RP1 & \multirow{9}{*}{1.0} & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP2 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP3 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP4 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.98 \\
& RP5 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.96 \\
& SICO &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 \\
& RB &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.99 & 0.99 & \\
& SCTS &  & 1.0 & 1.0 & 1.0&1.0 & 0.98 & 0.94 & 0.67 & 0.66 & 0.66 & 0.66 & \\
& Oracle &  & 1.0 & 1.0 & 1.0 & 0.99 & 0.86 & 0.4 & 0.07 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 5
\multirow{9}{*}{5} 
& RP1 & \multirow{9}{*}{1.0} & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP2 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
& RP3 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.95 \\
& RP4 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.95 \\
& RP5 &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.94 \\
& SICO &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 \\
& RB &  & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & \\
& SCTS &  & 1.0 & 1.0 & 1.0 & 0.95 & 0.9 & 0.83 & 0.52 & 0.49 & 0.49 & 0.49 & \\
& Oracle &  & 1.0 & 1.0 & 1.0 & 0.80 & 0.35 & 0.01 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}



\begin{table*}[!t]
\centering
\caption{Success Rate table comparing different methods with budgets for selfhash.}
\label{tab:success_rate}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
c & Method & 0 (Unattacked) & 0.05 & 0.1 & 0.15 & 0.2 & 0.25 & 0.3 & 0.35 & 0.4 & 0.45 & 0.5 & 1.0 (Unconstrained) \\ 
\midrule
% c = 1
\multirow{3}{*}{1} 
& SCTS & 0.8 & 0.7 & 0.2 & 0.2 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
& RB & 0.8 & 0.8 & 0.7 & 0.4 & 0.3 & 0.3 & 0.3 & 0.2 & 0.1 & 0.1 & 0.1 & \\
& Oracle & 0.8 & 0.3 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 3
\multirow{3}{*}{3} 
& SCTS & 1.0 & 1.0 & 0.9 & 0.7 & 0.5 & 0.3 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & \\
& RB & 1.0 & 1.0 & 1.0 & 1.0 & 0.9 & 0.7 & 0.7 & 0.7 & 0.6 & 0.5 & 0.2 & \\
& Oracle & 1.0 & 1.0 & 0.8 & 0.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 4
\multirow{3}{*}{4} 
& SCTS & 1.0 & 1.0 & 0.9 & 0.5 & 0.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
& RB & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.8 & 0.9 & 0.7 & 0.5 & 0.5 & 0.5 & \\
& Oracle & 1.0 & 1.0 & 0.7 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\midrule
% c = 5
\multirow{3}{*}{5}
& SCTS & 1.0 & 0.89 & 0.89 & 0.78 & 0.11 & 0.11 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
& RB & 1.0 & 1.0 & 1.0 & 1.0 & 0.89 & 0.89 & 0.78 & 0.67 & 0.56 & 0.33 & 0.33 & \\
& Oracle & 1.0 & 1.0 & 0.67 & 0.22 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> contents/deprecated.tex <==
\subsection{old}


\varun{first, state the lemma's objective in words.}

\ql{The important point is not the conclusion, is rather we can use this to analyze previous methods and SCTS}
\task{need one more rewrite}

Under the assumption that the $c+1$-grams are $i.i.d.$ green with probability $q$, then we have results depending on if $q>\gamma$.

Recall
$$z = \frac{\|T\|_G - \gamma T_e}{\sqrt{T_e \gamma (1 - \gamma)}}$$
When $\|T\|_G\sim B(T_e,q)$, then
$$\mathbb{E}[z] =\frac{q-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e}$$
\subsubsection{$q>\gamma$}
$$\mathbb{E}[z] \propto \sqrt{T_e}.$$

Let $$\mathbb{E}[z] = z_{th},$$ then $$T_c=\frac{\gamma(1-\gamma)z_{th}^2}{(q-\gamma)^2}.$$

Let us denote $C_\gamma=\sqrt{\gamma(1-\gamma)}$ for more clear notation.
When $T_e\geq T_c$, the probability of being detected as unwatermarked can be upper-bounded using the Chernoff bound of the binomial distribution. 
\begin{align*}
P(z \leq z_{th}) &= P(\|T\|_G \leq C_\gamma z_{th} + \gamma T_e) \\
                 &\leq \exp\left(-T_eD\left(\frac{C_\gamma z_{th}}{T_e}+\gamma || q \right)\right),
\end{align*}

where $$D(a||q)$$ is KL-divergence with base $e$:
$$D(a||q)\coloneqq a \ln \frac{a}{q}+(1-a)\ln{\frac{1-a}{1-q}}$$


\noindent{\bf Conclusion}
When $q>\gamma$, sufficiently long text will be detected as watermarked with high probability.
\subsubsection{$q<\gamma$}
$$\mathbb{E}[z] \propto -\sqrt{T_e}.$$
$T_c$ does not exist.
The detection the probability to be detected as unwatermarked can be upper-bounded similarly.
\begin{align*}
P(z > z_{th}) &\leq P(z \geq z_{th}) \\
              &= P(\|T\|_G \geq C_\gamma z_{th} + \gamma T_e) \\
              &\leq \exp\left(-T_eD\left(\frac{C_\gamma z_{th}}{T_e}+\gamma || q \right)\right) \\
              &< \exp\left(-T_eD(\gamma || q)\right),
\end{align*}


\noindent{\bf Conclusion}
When $q<\gamma$, the probability to be detected as unwatermarked converge to $0$ fast.
\subsubsection{$q=\gamma$}
$$\mathbb{E}[z] = 0$$
(De Moivre–Laplace theorem)
When $T_e \to \infty$, the distribution of $z$ approaches the normal distribution $N(0,1)$. The probability of detected as watermarked
$$
P(z>z_{th}) \to 1-\Phi(z_{th})
$$

\subsection{\bf Why Existing Methods do not Work for Long Text}

%\noindent{\bf Scalibility}

%\varun{what is a c-gram?} 
%\ql{left (self) hash: current token + c (c-1) tokens to the left. Kind of oversimplifying. Will add explanation to left / self hash}

\varun{write some text here on (a) what the objective of this section is, and (b) how we are going to come to a conclusion of this objective based on the math below}

In this subsection, we will see that existing color-agnostic methods are likely to only dilute the watermark in the watermarked text, which remain detectable when the text is sufficiently long. We will use the above lemma to see how they fail.

\subsubsection{Unattacked Text}

\varun{need some explanation here on what you are doing, and what you hope to achieve}

%$$z = \frac{\|T\|_G - \gamma T_e}{\sqrt{T_e \gamma (1 - \gamma)}}$$
Note that $p>\gamma$, apply the lemma ($q=p>\gamma$)
%$$\|T\|_G\sim B(T_e,q)$$

%$$\mathbb{E}[z] = \frac{p T_e- \gamma T_e}{\sqrt{T_e \gamma (1 - \gamma)}}=\frac{p-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e}$$
Watermark strength
$$\mathbb{E}[z] =\frac{q-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e} \propto \sqrt{T_e}.$$
Critical length
$$T_c=\frac{\gamma(1-\gamma)}{(p-\gamma)^2}z_{th}^2$$
False negative rate is upper-bounded 
\begin{align*}
P(z \leq z_{th}) &\leq \exp\left(-T_eD\left(\frac{C_\gamma z_{th}}{T_e}+\gamma || p \right)\right),
\end{align*}

\begin{comment}
From Hoeffding's inequality, we have
$$\Pr(\|T\|_G \leq r)\leq \exp(-2T_e(p-\frac{t}{T_e})^2)$$
for $t\leq \mathbb{E}[\|T\|_G]=pT_e$.

\vspace{2mm}

When $T_e \geq T_c $, let $t=z_{th} \sqrt{\gamma(1-\gamma)T_e}+\gamma T_e \leq pT_e$.
\begin{align*}
&\Pr(z \leq z_{th}) \\
\leq& \exp\left(-2\left((p-\gamma)\sqrt{T_e}-z_{th}\sqrt{\gamma(1-\gamma)}\right)^2\right) \\
=& \exp\left(-2(p-\gamma)^2\left(\sqrt{T_e}-\sqrt{T_c}\right)^2\right)
\end{align*}

%\ql{right-hand size is "critical length"}
 this probability of unsuccessful detection will go to $0$ fast as $T_e$ increases.




\ql{remove standard deviation as it is not necessary. standard deviation is useful if we use Chebyshev inequality, yet may be looser. Wikipedia mentions alternative tighter bounds for binomial distribution}
%Standard deviation
%$$\sigma_z=\sqrt{\frac{\Pr(1-p)}{\gamma(1-\gamma)}}$$ is a constant.

\varun{$\mathbb{E}[z] = z$?} \ql{previously I directly used z, which is not mathematically correct}
\end{comment}
\noindent{\bf Conclusion}
Watermark strength $\mathbb{E}[z]\propto \sqrt{T_e}$. The probability of false negative converges to $0$ expoentially w.r.t. $T_e$.

\subsubsection{Attack 1}
\ql{We can simplify this as the derivation is trivial}
\varun{need some explanation here on what you are doing, and what you hope to achieve}
There are attacks like designing prompts to guide the watermarked model to generate low-entropy texts to evade detection, where it is harder to incorporate watermarks into more deterministic texts. However, we will see that it may only dilute the watermark.

Assume the attacker can reduce $p$ to $p'$, but $p'>\gamma$, i.e., the $c+1$-grams are $i.i.d.$ green with probability $p'$, then we have results depending on if $p'>\gamma$.
Then the above still holds except we use $p'$ instead of $p$.

Watermark strength
$$\mathbb{E}[z] =\frac{p'-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T}$$
New critical length
$$T_c'=\frac{\gamma(1-\gamma)}{(p'-\gamma)^2}z_{th}^2$$
The probabilty of evading the attack converge to $0$ exponentially w.r.t. $T_e$. 
\begin{align*}
P(z \leq z_{th}) &\leq \exp\left(-T_eD\left(\frac{C_\gamma z_{th}}{T_e}+\gamma || p \right)\right),
\end{align*}
%\begin{align*}
%&\Pr(z \leq z_{th}) \\
%\leq& \exp\left(-2\left((p'-\gamma)\sqrt{T_e}-z_{th}\sqrt{\gamma(1-\gamma)}\right)^2\right) \\
%=& \exp\left(-2(p'-\gamma)^2\left(\sqrt{T_e}-\sqrt{T_c'}\right)^2\right)
%\end{align*}

\noindent{\bf Conclusion}
This attack would fail for sufficiently long watermarked text because it can only dilute the watermark.

\subsubsection{Attack 2}
In this attack, the attacker is using color-agnostic post-processing methods, i.e., color-agnostic post-processing is applied to watermarked text to evade detection. Existing paraphrasing-based methods \citep{lu2023large, krishna2023paraphrasing} fall into this category. We will see these methods still can only dilute the watermark.
%We assume the post-processed text includes two parts of $c+1$-grams.
%$$0 < \mathbb{E}[z'] =\frac{p'-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T}\propto \sqrt{T}$$, and standard deviation is still a constant $$\sigma_z'=\sqrt{\frac{p'(1-p')}{\gamma(1-\gamma)}}$$. Then this method would fail for sufficiently large $T$. This corresponds to the result in \citet{kirchenbauer2023reliability}. 

\varun{need some explanation here on what you are doing, and what you hope to achieve}


\noindent{\bf Assumptions}
\begin{itemize}
    \item The post-processing is color-agnostic. We assume the new $c+1$-grams are green with i.i.d. probability $\gamma$, and the number of such new $c+1$-grams is $T_{n}$. We call them new $c+1$-grams.
    \item Postprocessing like paraphrasing is statistically likely to leak n-grams or even longer fragments of the original text \citep{kirchenbauer2023reliability}. We call them old $c+1$-grams. These old $c+1$-grams are green with i.i.d. probability $p$ from the previous assumption, and the number of such old $c+1$-grams is $T_{o}$. 
    \item The above two composes post-processed text's $c+1$-grams, implying $T_e=T_o+T_n$.
    \item Assume $c+1$-gram leaking ratio $r_o=\frac{T_o}{T_o+T_n}$, is a constant independent from $T_o+T_n$.
\end{itemize}
We have 
\begin{align*}
\mathbb{E}[z] &= \gamma = \frac{(T_n \gamma + T_o p) - \gamma(T_o + T_n)}{\sqrt{(T_o + T_n)\gamma(1 - \gamma)}} \\
       &= \frac{p - \gamma}{\sqrt{\gamma(1 - \gamma)}} r_o \sqrt{T_e} \\
       &\propto \sqrt{T_e}
\end{align*}

%$$\sigma_{z''}=\sqrt{\frac{\gamma(1-\gamma)(1-r_o)+\Pr(1-p)r_o}{\gamma(1-\gamma)}}$$ is a constant.
\noindent{\bf Definition}
\begin{itemize}
    \item $\|T\|_G^o$: the number of green old $c+1$-grams as a random variable
    \item $\|T\|_G^n$: the number of green new $c+1$-grams as a random variable
\end{itemize}
So $\|T\|_G^o\sim B(T_o,p)$, $\|T\|_G^n\sim B(T_n,\gamma)$, $\|T\|_G=\|T\|_G^o+\|T\|_G^n $. \ql{No longer binomial here. We may use Chernoff bound but keep it simple for now.}

New critical length
$$T_c'=\frac{\gamma(1-\gamma)}{r_o^2(p-\gamma)^2}z_{th}^2$$
From Hoeffding's inequality, we have 
$$\Pr(T_op+T_n\gamma-\|T\|_G \leq t)\leq \exp (-\frac{2t^2}{T_o+T_n})$$
for $t\geq0$.

When $T_o+T_n\geq T_c'$, take
$$t=T_o(p-\gamma)-z_{th}\sqrt{\gamma(1-\gamma)(T_o+T_n)} \geq 0,$$
then
\begin{align*}
&\Pr(z \leq z_{th}) \\
\leq& \exp\left(-2\left(r_o(p-\gamma)\sqrt{T_e}-z_{th}\sqrt{\gamma(1-\gamma)}\right)^2\right) \\
=& \exp\left(-2r_o^2(p-\gamma)^2\left(\sqrt{T_e}-\sqrt{T_c'}\right)^2\right)
\end{align*}

Still, the probability to evade detection expoentially converge to $0$ w.r.t. $T_e$.

\noindent{\bf Remark}
In paraphrasing, we can safely assume when the watermarked text being paraphrased becomes longer, the paraphrased text becomes longer accordingly.

\noindent{\bf Conclusion}
This attack would fail for long enough generated text when a non-zero ratio of $c+1$-grams is preserved. % need to be more precise here
%More specifically: 
%\ql{add argument computing standard deviation here}

\noindent{\bf Remark}
Even if attack 1 and attack 2 are combined, i.e., the attacker can let the watermarked text be weaker and do color-agnostic post-processing, then it would still fail for sufficiently long text. To see this, just let $p=p'>\gamma$ in the above derivation.

\ql{1/30: ends here}

\subsubsection{\bf Color-agnostic Substitution Baseline - an implementation of attack 2}
\noindent{\bf Assumption}
For simplicity, we assume $c=1$. Then $c+1$-grams are $2$-grams, $T_e=T-1$. This assumption is for all remaining parts of this section.

If we substitute \( s^{(t)} \) with \( s_n^{(t)} \), then the color of 2 new $2$-grams $(s^{(t-1)},s_n^{(t)})$ and $(s_n^{(t)},s^{(t+1)})$ may change. If this is color-agnostic, it is reasonable to assume all those new $2$-grams are green with i.i.d. probability $\gamma$. 
%The expectation of green tokens for these two before replacement is \( 2p \), and after is \( 2\gamma \).
We do \( \frac{kT_e}{2} \) replacements (non-adjacent and only for tokens starting from the second) in a string of \( T \) tokens. 
Then this goes to the attack 2 case, $T_o=(1-k)T_e$, $T_n=kT_e$, $r_o=1-k$

\begin{align*}
\mathbb{E}[z]  &= \frac{p - \gamma}{\sqrt{\gamma(1 - \gamma)}} (1-k) \sqrt{T_e} \\
\end{align*}

New critical length
$$T_c'=\frac{\gamma(1-\gamma)}{(1-k)^2(p-\gamma)^2}z_{th}^2$$

\begin{align*}
&\Pr(z \leq z_{th})\\
=& \exp\left(-2(1-k)^2(p-\gamma)^2\left(\sqrt{T_e}-\sqrt{T_c'}\right)^2\right)
\end{align*}


%As the case for existing color-agnostic paraphrasing methods,
%\begin{align}
%0 \leq \mathbb{E}[z'] &= \frac{\|T\|_G  - 2(p-\gamma)\frac{kT}{2}- \gamma T}{\sqrt{\gamma(1-\gamma)T}} \nonumber \\
%&= \frac{(1-k)(p-\gamma)}{\sqrt{\gamma (1-\gamma)}}\sqrt{T} \propto \sqrt{T}
%\end{align}
%$$\sigma_{z''}=\sqrt{\frac{\gamma(1-\gamma)k+\Pr(1-p)(1-k)}{\gamma(1-\gamma)}}$$ is a constant give k.
%We need to (almost) replace one token for every two tokens (e.g., 2nd, 4th, 6th, ...).

\noindent{\bf Conclusion}: Approximately \( \frac{T_e}{2} \) replacements are necessary to evade detection, meaning all $2$-grams are new to be scalable to arbitiarily long texts. If not, watermarking is only diluted. % In the sense of watermark detection this is equivalent to paraphrasing.

\subsection{\bf Color-aware Substitution}
% our method is far from this, may remove later
We can have a similar analysis assuming non-adjacent color-aware substitutions. The expectation of green $2$-grams for these two before the substitution is \( 2p \),  after is $0$. If we do \( \frac{kT}{2} \) replacements (non-adjacent) in a string of \( T \) tokens, then:
\begin{align*}
\mathbb{E}[z] &= \frac{\|T\|_G - 2p\frac{kT_e}{2} - \gamma T_e}{\sqrt{\gamma(1-\gamma)T_e}} \\
      &= \frac{(1-k)p - \gamma}{\sqrt{\gamma (1-\gamma)}}\sqrt{T_e}
\end{align*}
%$$
%\sigma_{z''}=\sqrt{\frac{\Pr(1-p)(1-k)}{\gamma(1-\gamma)}}
%$$
%is a constant given $k$
Let $\mathbb{E}[z]\leq 0$, we have $k\geq 1-\frac{\gamma}{p}\coloneqq k_c$. 

Critical ratio $k_c$ is a rough lower-bound for the number of substitutions needed.

\ql{argument using Hoeffding to bound the probability}
$T_o=(1-k)T_e$, $T_n=kT_e$.
As for critical length, let $\mathbb{E}[z]=z_{th}$
$$T_c=\frac{\gamma(1-\gamma)}{((1-k)p-\gamma)^2}z_{th}^2, 0\leq k < k_c $$
and do not exist for $k \geq k_c$. 

Then we will bound the probability that the attack fails to evade watermark detection.

When $k \geq k_c$, let
\begin{itemize}
    \item $\|T\|_G^o$: the number of green old $c+1$-grams as a random variable
    \item $\|T\|_G^n$: the number of green new $c+1$-grams as a random variable
\end{itemize}
So $\|T\|_G^o\sim B((1-k)T_e,p)$, $\|T\|_G^n=0$.
From Hoeffding's inequality, we have 
$$\Pr(\|T\|_G -(1-k)pT_e \geq t)\leq \exp(-\frac{2t^2}{(1-k)T_e})$$
for $t\geq0$.

Let $t=z_{th}\sqrt{\gamma(1-\gamma)T_e}+(\gamma-(1-k)p)T_e\geq z_{th}\sqrt{\gamma(1-\gamma)T_e} \geq 0$.

Then 
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2 \left( (\gamma-(1-k)p)\sqrt{T_e} + \frac{\sqrt{\gamma(1-\gamma)}}{\sqrt{1-k}}z_{th} \right)^2 \right)
\end{align*}

\noindent{\bf Case 1}: $k=k_c$
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2 \frac{\gamma(1-\gamma)}{1-k}z_{th}^2 \right)
\end{align*}
This is a constant bound.
\ql{A tighter bound may show it converges to zero (minor).}

\noindent{\bf Case 2}: $k>k_c$
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2(\gamma-(1-k)p)^2 \right. \\
\qquad& \times \left. \left( \sqrt{T_e} + \frac{\sqrt{\gamma(1-\gamma)}}{\sqrt{1-k}(\gamma-(1-k)p)}z_{th} \right)^2 \right)
\end{align*}
converge to $0$ fast as $T_e$ increases when $k$ is fixed.
\noindent{\bf Conclusion}: When $k>k_c=1-\frac{\gamma}{p}$, then $E(z)\propto -\sqrt{T_e}$, probability such attack fails to converge to zero fast as the length increases, i.e., the attack is successful and scalable for arbitrarily long text. 

\newpage

\ql {special above. $0$ probability give tighter bounds}

\subsection{\bf More General Color-aware Substitution}

\noindent{\bf Assumption 1}
For simplicity, we assume $c=1$. Then $c+1$-grams are $2$-grams, $T_e=T-1$. This assumption is for all remaining parts of this section.

\begin{itemize}
    \item $T_o$: number of old $c+1$-grams in the attacked text
    \item $\|T\|_G^o$: the number of green old $c+1$-grams as a random variable
    \item $T_n$: number of new $c+1$-grams in the attacked text
    \item $\|T\|_G^n$: the number of green new $c+1$-grams as a random variable
\end{itemize}

\noindent{\bf Assumption 2}
New $c+1$-grams are green with probability $p_n<p$, $i.i.d.$.

$\|T\|_G^o\sim B(T_e,p)$, $\|T\|_G^n\sim B(T_e,\gamma)$.
From Hoeffding's inequality, we have 
$$\Pr(\|T\|_G -(1-k)pT_e \geq t)\leq ex\Pr(-\frac{2t^2}{(1-k)T_e})$$
for $t\geq0$.

Let $t=z_{th}\sqrt{\gamma(1-\gamma)T_e}+(\gamma-(1-k)p)T_e\geq z_{th}\sqrt{\gamma(1-\gamma)T_e} \geq 0$.

Then 
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2 \left( (\gamma-(1-k)p)\sqrt{T_e} + \frac{\sqrt{\gamma(1-\gamma)}}{\sqrt{1-k}}z_{th} \right)^2 \right)
\end{align*}

\noindent{\bf Case 1}: $k=k_c$
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2 \frac{\gamma(1-\gamma)}{1-k}z_{th}^2 \right)
\end{align*}
This is a constant bound.
\ql{A tighter bound may show it converges to zero (minor).}

\noindent{\bf Case 2}: $k>k_c$
\begin{align*}
&\Pr(z \geq z_{th})\\
\leq& \exp \left( -2(\gamma-(1-k)p)^2 \right. \\
\qquad& \times \left. \left( \sqrt{T_e} + \frac{\sqrt{\gamma(1-\gamma)}}{\sqrt{1-k}(\gamma-(1-k)p)}z_{th} \right)^2 \right)
\end{align*}
converge to $0$ fast as $T_e$ increases when $k$ is fixed.
\noindent{\bf Conclusion}: When $k>k_c=1-\frac{\gamma}{p}$, then $E(z)\propto -\sqrt{T_e}$, probability such attack fails to converge to zero fast as the length increases, i.e., the attack is successful and scalable for arbitrarily long text. 

\newpage
\subsection{Our Approach: Self Color Testing (SCT)}

\noindent{\bf Key Insight}
The key for successful attack against watermarked LLM is to have color information. This is not easy, but we can do by prompting the model to generate random string, and infer color information from the frequency.

We makes the following adaptation for prompting:  
\begin{itemize}
\item We work on word-level to avoid some encoding issues and incomplete word biases.
\end{itemize}

\begin{algorithm}
\SetAlgoLined % This sets line numbering on, but you can remove it if you don't want line numbers
\textbf{Input:} $w_b$, $w_b'$, $w_b^c=w_{b-c}\ldots w_{b-1}$\;
\textbf{Output:} Test result in $\{GR,RG,S\}$. $GR$ ($RG$) means $w_b$ is green (red) while $w_b'$ is red (green)\;

$p=\text{prompt}(w_b, w_b', w_b^c)$\;
$text=\text{LLM}(p)$\;
$c_b, c_b' = \text{count}(text, w_b^cw_b), \text{count}(text, w_b^cw_b')$\;
$p_t=\chi^2\text{-test}(c_b, c_b')$\;
  \If{$p_t \geq p_{th}$}{
    \Return $S$\;
    }
    \uElseIf{$c_b>c_b'$}{
    \Return $GR$\;
    }
    \Else{
    \Return $RG$\;
    }
\caption{Self Color Testing}
\end{algorithm}

We make further assumptions for the ease of understanding:


\noindent{\bf Assumptions}
\begin{enumerate}
    \item Temperature $t=0$, meaning deterministic generation from probabilities.
    \item The LLM's random generation follows the prompt's instruction.
\end{enumerate}

And our example prompt for color testing is as follows $(w_b=includes, w_b'=contains, w_b^c=kernel)$:
Choose two phrases ( kernel includes, kernel contains ), and generate a long uniformly random string of those words separated by ";". Previous phrases should have no influence on future phrases: kernel includes; kernel contains; kernel includes; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains;

Here the word "includes" is the word being substituted, "contains" is the candidate word. Then we check the frequency of the response for this prompt.

Assume the token before "includes" and "contains" are the same in the encoded "kernel includes" and "kernel contains". 
%\begin{itemize}
%    \item Do a $\chi^2$ test.
%    \item If p-value $\geq$ threshold, then we conclude they are both green or both red.
%    \item If p-value < threshold, then the lower frequency one is red and the higher one is green.
%\end{itemize}
Then as the model is determinsitic, and the model follows the prompt's probablity, then the model will always generate the green one if $w_b$ and $w_b'$ are of different colors, so SCT has perfect recall on $GR$ and $RG$. For $S$ there can be border cases but in realistic applications, $t>0$ so they will have the same probability to appear. 

\noindent{\bf SCTS}
The idea is to use color-testing to test different candidates to try to ensure that the token is substituted from green to red.
\noindent{\bf Algorithm}

\begin{algorithm}
\SetAlgoLined % This sets line numbering on, but you can remove it if you don't want line numbers
\textbf{Input:} $w$, \\
\textbf{Output:} $w'$\\
\textbf{Initialization:} $i=c$, $w'=w$\\
\While{$i \leq n$}{
    $w_{b1},\ldots,w_{bk} = \text{generate\_candidates}(w', i)$\\
    $success=\text{False}$\\
    \For{$j=1$ \KwTo $k$}{
        \If{$\text{SCT}(w_i, w_{bj}, w_{i-c}\ldots w_{i-1}) == \text{GR}$}{
            $w'=\text{Substitute}(w',i,w_{bj})$\\
            $success=\text{True}$\\
            break
        }
    }
    \eIf{success}{
        $i\gets i+2$\\ advance by 2 for economic substitution
    }{
        $i\gets i+1$\\
    }
}
\caption{SCTS Algorithm}
\end{algorithm}
\noindent{\bf Budget enforcement}
To enforce budget, we add checking if the budget is reached after each replacement based on the previous SCTS.

\subsection{\bf SCTS analysis}

\noindent{\bf Success Probability}
For the success probability for each attempt with $k$ candidates
\begin{equation}
    p_s = (1-\gamma^k)p
\end{equation}
\noindent{\bf Expected Green Ratio}
%Have not figured out how to compute the expectation of the number of green tokens after replacement. Yet this is stronger than Scheme 1 without additional computation (for each replacing attempt).
We make the following assumptions:
\begin{itemize}
    \item $c=1$
    \item One token per word for simplicity (or token-level attack)
    \item Candidate generation process is independent from red and green list, i.e., every candidate is green with $i.i.d.$ probability $\gamma$
\end{itemize}

To figure out the estimated expected ratio $r_g^T=\mathbb{E}[\|T\|_G]/T_e$ of green $2$-grams after SCTS attack, we need some mathematics.

Let the expected number of green $2$-grams after SCTS attack (for $T_e$ $2$-grams) be $e_{T_e}$. Let $p_s$ be the probability of successful substitution for the first $2$-gram. Let $e_2'$ be the expected number of green $2$-grams in the first two $2$-grams when the attempt to substitute the first $2$-gram is successful. Let $e_1'$ be the expectation of the number of green $2$-gram when the attempt to substitute the first $2$-gram is not successful. Then we have:
\begin{equation}
e_T = p_s(e_{T_e-2} + e_2') + (1-p_s)(e_{T_e-1} + e_1')
\end{equation}

We have
\begin{multline}
T_e \cdot r_g^{T_e} = p_s(r_g^{T_e-2} \cdot (T_e-2) + e_2') \\
+ (1-p_s)(r_g^{T_e-1} \cdot (T_e-1) + e_1')
\end{multline}

Let $r_g = \lim_{T_e \to \infty} \frac{e_T}{T_e}$,  $T_e \to \infty$, then

\begin{multline}
T_e \cdot r_g = p_s(r_g \cdot (T_e-2) + e_2') \\
+ (1-p_s)(r_g \cdot (T_e-1) + e_1')
\end{multline}
\begin{equation}
r_g = \frac{p_s e_2' + (1-p_s)e_1'}{1 + p_s}
\end{equation}
We have
\begin{align*}
p_s &= \Pr(1-\gamma^k), \\
e_2' &= \gamma, \\
e_1' &= \Pr(\text{$2$-gram being green} | \text{attempt fails}) \\
&= \Pr(\text{attempt fails} | \text{$2$-gram being green})\\
&\cdot \Pr(\text{$2$-gram being green}) / \Pr(\text{attempt fails}) \\
&= \frac{\gamma^k \cdot p}{1-p_s}.
\end{align*}
Plug in:
\begin{equation}
r_g - \gamma = -\frac{\gamma(1-p\gamma^{k-1})}{1+\Pr(1-\gamma^k)} < 0
\end{equation}
(and the right hand size is a constant).

\begin{align*}
\mathbb{E}[z] &= \frac{r_g T_e - \gamma T_e}{\sqrt{T_e \gamma (1 - \gamma)}} \\
     &= \frac{r_g - \gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e} \\
     &= -\frac{\gamma(1-p\gamma^{k-1})}{(1+\Pr(1-\gamma^k))\sqrt{\gamma(1-\gamma)}}\sqrt{T_e} \\
     &\propto -\sqrt{T_e}
\end{align*}

When $k \to \infty$, $r_g - \gamma \to -\frac{\gamma}{1+p}$, 
\begin{align*}
\mathbb{E}[z] = -\frac{\gamma}{(1+p)\sqrt{\gamma(1-\gamma)}}\sqrt{T_e}
\end{align*}

\task{before here, introduce a more general substitution-based attack, then ideal and this are all special case}
%So we can see that in expectation SCTS can reduce green list ratio to less than $\gamma$ with a constant margin so it is scalable to arbitrarily large $T_e$.

\ql{tried but did not find a way to bound the standard deviation}

\noindent{\bf LLM Call Expectations}
As \( T_e \to \inf \), the expected number of LLM calls per attempt can be calculated. This is crucial for scaliability. Let the expectation of LLM calls be \( n_T \). Let the expected ratio of LLM calls be \( y_T = \frac{n_T}{T} \). Let \( y = \lim_{T \to \infty} \frac{n_T}{T} \).
\begin{equation}
    y = \frac{p\gamma + (1-p)(1-\gamma)}{(1+p)\gamma(1-\gamma)}
\end{equation}
For example, with \( p=0.5 \) and \( \gamma=0.25 \), this value is \( \frac{16}{9} \).

\noindent{\bf Derivation}

\begin{align}
n_T &= \sum_{i=1}^{m} \Pr(\text{success at the } i\text{-th time}) (n_{T-2} + i) \nonumber \\
    &\quad + (1 - p_s)(n_{T-1} + n_1')
\end{align}
 Let \( T \to \infty \), \( N_1' \) denotes the number of calls when there is no success with expectation \( n_1' \) for the first attempt
\begin{align}
Ty &= \sum_{i=1}^{k} \Pr(\text{success at the } i\text{-th time})((T-2)y + i) \nonumber \\
   &\quad + (1-p_s)((T-1)y + n_1')
\end{align}


\[
y = \frac{\sum_{i=1}^{k} i \Pr(\text{success at the } i\text{-th time}) + (1-p_s)n_1'}{1 + p_s}
\]
From this, we can get \( y \) for any \( k \), but the math is cumbersome. For simpler math, let \( k \to \infty \)
Then \( p_s = p \), \( N_1' \) is a geometric distribution with mean \( n_1' = \frac{1}{\gamma} \), 
\[
\Pr(\text{success at the } i\text{-th time}) = p \gamma^{i-1} (1-\gamma)
\]
so
\[
\sum_{i=1}^{\infty} i \Pr(\text{success at the } i\text{-th time}) = \frac{p}{1-\gamma}
\]
Plug in
\[
y = \frac{p \gamma + (1-p)(1-\gamma)}{(1+p) \gamma (1-\gamma)}
\]


==> contents/guidelines.tex <==
How to improve paper writing ability?
What is your previous experience?
Answer changes depending on writing an ML paper vs. Security/Systems paper.
Format below is common, but level of detail will change.
Security conferences allow 13 pages, double column.
Can write more text here.
Expect more clarity and precision.
ML conferences allow 9 pages, single column.
Expect more communication of main ideas and evaluation of main ideas.
Details are often punted to the appendix.
Always follow the formula below:
Section 0: Abstract
Think of this as an elevator pitch for your paper.
Should be less than 10-12 sentences in total.
Should answer the same questions as in the introduction, but more concisely. 
Section 1: Introduction
Introduction should give the reader some broader context of the problem
It should usually be 1-1.5 pages in length
Introduction should contain a summary of the paper: it should answer the following questions
Why is the problem being solved important?
What did previous solutions to the problem do, and where did they fail?
What is your solution doing that is better than previous works?
How did you evaluate it + what are your takeaways from evaluation?
A bullet point list of the main contributions of the paper
<always write the introduction last, after writing other sections of the paper. That way, you’ll know what is in the paper, and you can modify the introduction and the answer to the above questions accordingly>
Section 2: Notation to be used in the paper
Being precise about mathematical formulation is VERY IMPORTANT!!!!
It is more professional + always more reproducible if the math is correct
Section 3: Motivation for the problem being solved + preliminary experimental evidence to support motivation
Section 4: Main technical contributions
Always motivate your contribution using 1 or 2 strawmen solutions (i.e., solutions for the problem that are not that good)
The strawmen solutions should give “suggestive information” on how to design more optimal solutions.
Section 5: Experimental setup
Should contain a link to any open source code that you are releasing as part of your work
Section 6: Experimental evidence for your technique
Always follow a format where you ask “THREE” main questions that you want to answer
Each answer should be in one individual subsection
Format can be found in https://arxiv.org/pdf/1912.03817.pdf (as an example)
Section 7: Discussion & other open questions
Section 8: Related work
Section 9: Conclusions


==> contents/notations.tex <==
\newpage
\section{Notations}
\label{sec:notation}

\varun{this can be merged with section 2.1 i.e., watermarking approaches}

\varun{if the notations is being borrowed from a different paper, please be sure to state that up front!}
\ql{what do we need to list here? all or only important ones (not those only appear in the proof?) } \varun{important ones + what we need in the proof}

The notations used in this paper are partly borrowed from \citep{kirchenbauer2023watermark} and \citep{kirchenbauer2023reliability}. For clarity and ease of understanding, we list the key notations below, focusing on those that are crucial for understanding the main text and our proofs.

\begin{itemize}
\item $z$: Score used for watermark detection.
\item $z_th$: Detection threshold
\item $T$: Total number of tokens in the (tokenized) sample (text sent to the detector).

\item $T'$: Total number of words in the sample (text sent to the detector). %Note: It's important to clarify the distinction between 'tokens' and 'words' in this context.
\item $\|s\|_G$: Number of green tokens in the sample.
\item $\gamma$: Proportion of green tokens in the vocabulary.
\item $p$: Assumed uniform probability of a token being green in the watermarked text.
\item $w = w_0,w_1,\cdots,w_{T'-1}$: Sequence representing the watermarked text, where each $w_i$ is a word.
\item $k$: Number of candidate substitutions.
\item $w_b$: Word in the text being considered for substitution.
\item $w_b'$: Candidate substitution word for $w_b$.
\item $c$: Context width, used in defining the local context for a substitution.
\item $w_b^c$: Local context of $w_b$, defined as $w_b^c = w_{b-c}...w_{b-1}$, representing the $c$ words preceding $w_b$.
\item $p_t$: p-value in hypothesis testing, used for statistical decision-making.
\item $p_{th}$: Threshold for the p-value for $\chi^2$-test, determining the significance level in hypothesis testing.
\item $t$: Temperature parameter in LLM decoding, influencing the randomness in token generation.
\item $\delta$: Bias introduced in the probability distribution due to watermarking.
\item $T_e$:
\item $c+1$-gram
\end{itemize}

==> contents/results/result_2.tex <==
\subsection{\bf General Substitution}
%\ql{problem: this extension does not hold for our attack, and only applied once besides the removed hypothetical color-aware attack, making it not so useful}

\noindent{\bf Assumption 1}
For simplicity, we assume $c=1$. Then $c+1$-grams are $2$-grams, $T_e=T-1$. Larger $c$ are essentially similar. This assumption is for all remaining parts of this section.

% our method is far from this, may remove later
We have shown the weakness of color-agnostic methods. Let $0<r_n\leq 1$ be constant independent from $T_e$. Assume we have made $\frac{r_n T_e}{2}$ non-adjacent substitutions. To maximize the number of new $2$-grams given fixed number of substitutions, as one substitution changes up to two $2$-grams, we assume exactly two for simplicity. 

\varun{what is $r_n$ and $p_n$ and $p_o$? is $r_n$ some random constant? }
\noindent{\bf Grouping}
We divide $r_n T_e$ new $2$-grams to $\frac{r_n T_e}{2}$ 2-group, where $2$-grams are in the same group $\iff$ they are new because of the same substitution. The old $2$-grams are grouped in one $2$-gram one-group manner. \label{GeneralGrouping}

\noindent{\bf Assumption 2}
\begin{itemize}
    \item The number of green $2$-grams in each new $2$-gram group (two $2$-grams) are random variables with expectation $2p_n$.
    \item The number of green $2$-grams in each old $2$-gram group (one $2$-gram) are random variables with expectation $p_o$.
    \item The number of green $2$-grams of different groups are independent.
\end{itemize}

Average green probability $\overline{p}=r_n p_n+(1-r_n)p_o$. Even if the theorem cannot be directly applied, similar results can be derived. When $\overline{p}>\gamma$, the probability to evade watermarking exponentially converges to $0$ w.r.t. $T_e$; when $\overline{p}<\gamma$, the probability of failing to evade watermarking exponentially converges to $0$ w.r.t. $T_e$. More details are in the appendix. 

\noindent{\bf Conclusion} If substitution attacks can scale to arbitrarily long text depends on if the average green probability is at most $\gamma$.

\noindent{\bf {\bf Color-agnostic Substitution Baseline}}
From above, we do color-agnostic substitutions, so that we assume $p_n=\gamma$, $p_o=p$. Then $\overline{p}=r_n \gamma +(1-r_n)p \geq \gamma$. Consequently, unless $r_n=1$, the probability of evading watermarking exponentially converges to $0$ w.r.t. $T_e$. This implies almost at least half of the substitutions are required.

\ql{removed ideal color-aware substitution as it is not that ideal and important}




==> notes/attack.tex <==
\section{Attack}


\subsection{Repetitive String}

Assume $c$-grams, meaning that whether a token is green or red only depends on previous $c$ tokens. A repetitive string, like 'good good good ... good' (and each repetition unit is one token), is either all red or all green from the $c+1$-th token, and we call such repetitive ``red" or ``green," respectively. \textcolor{red}{VC: this is not true; the $c+1^{th}$ token (i.e., good) may be red or green (because it depends on the $c^{th}$ token), and the the $c+2^{nd}$ token (i.e., good) may be red or green (because it depends on the $c+1^{th}$ token, and these 2 are independent events. if you see algorithm 2, the vocabulary is divided for "each" token generation in a random manner}

\textcolor{blue}{Qilong: confirmed the repetitive string vulnerability claim by running the demo on Madison. }

\includegraphics[width=0.4\textwidth]{figures/good.png}


\includegraphics[width=0.4\textwidth]{figures/nice.png}

If we insert a repetitive string and the number of tokens is the same as the target text, then if such repetitive string is red, the red tokens will be roughly ($c$ is small) at least $50\%$ so the watermark detection fails. Note that if red tokens are significantly more than the green token, watermark detection will also fail as it is a one-sided test. If such repetitive sting is green, this attack will not work ($z$-score will be higher). The attack success rate will be $\approx50\%$ for a random token repeated in the repetitive string. \textcolor{red}{VC: i agree with the general premise that if the generation contains more red-tokens than green-tokens, the verification will fail. but this approach will not achieve that for the reasons mentioned. in fact, it is unclear how we can add only "red tokens" given that the color of the token depends on the key that is powered by all previous tokens}

\subsection{Hacking the Green and Red List}
\subsubsection{Assumptions}
\begin{enumerate}
    \item Temperature $t=0$, meaning deterministic generation from probabilities.
    \item The LLM's random generation follows the prompt's instruction.
    \item $c=1$ in $c-gram$
\end{enumerate}
\subsubsection{Color Test}
For ease of explanation, we assume that each word is tokenized to one token.
For example, we have a watermarked sample: `He is good.' \textcolor{red}{VC: what is the input? what is the generation?}
Just an example for watermarked text.
\newline
\newline
Craft such a prompt (inspired by Tang et al. ``Baselines for Identifying Watermarked Large Language Models"):
\newline
Generate a uniformly random string of ``good" and ``nice," but insert ``is" in between for each word for 1000 words. Previous string should have no influence on future string. \textcolor{red}{VC: could you elaborate please?}
\newline
\textcolor{blue}{Qilong: 
The prompt in Tang et al.: ``````Choose two digits, and generate a uniformly random string of those digits. Previous digits should have no influence on future digits:""" We specify the random token and add separators. 
} 


Then, from the second assumption, the word after "is" has an equal probability of being "good" and "nice" before the watermark. There will be three cases (their color if the previous word is ``is"): \textcolor{red}{VC: same problem as above; no uniformity since each token's color is independent}
\begin{enumerate}
    \item ``good" is green and ``nice" is red
    \item ``good" is red and ``nice" is green
    \item``good" and ``nice" are both green or both red
\end{enumerate}
For the first case, from the $t=0$ assumption, after ``is" it will always be ``good", because the probability of ``good" is boosted. For the second case, after ``is" it will always be ``nice". Both cases will give us a green-red pair. (The last case can also give us some color information.) Also, such color information can be reused.
\subsubsection{Replacement Attack}
Using the previous color test method, we can get the green-red pairs. The idea is to replace enough green words with red words.
\newline
\newline
For example, we do synonyms replacement for those which are green and red before and after replacement, respectively. Assume the probability of the new synonym to be green and red are equal. In each test, we have $\approx p/2$ probability on average of finding a green-red replacement, assuming the ratio of the green tokens in the target watermarked text is $p>1/2$ (for the case the watermark can be detected). We can try different synonyms for each word to be replaced and also try to replace different words. Replacing $p-1/2\leq 1/2$ of the tokens will ensure the red tokens are no less than the green, fail the watermarking detection. (Note that continuous replacement can change the context word.)
\subsubsection{Repetitive String Insertion Attack}
Using the previous color test method, we can also check if a repetitive string is red or green. This can be done by such a prompt:
\newline
Generate a uniformly random string of ``good" and ``nice" but insert ``good" in between for each word for 1000 words. Previous string should have no influence on future string.
\newline
So that the separator is ``good" instead of ``is". We can check how many words are ``good" and ``nice" at odd places from the 3rd place (3rd, 5th, etc.) now. Similarly, we can determine if the repetitive ``good" is green or red (equivalent to the color of the second ``good" in ``good good"). This test succeeds with probability $\approx1/4$, and we can try different words. After getting a red repetitive string, we can use that to attack. For stealthiness, we may use invisible tokens (if there are any) for the attack and may insert them in several places.
\subsection{Discussion}
Roughly speaking, for the color testing:
\newline
\begin{enumerate}
    \item Zero temperature assumption can be relaxed if we check frequency to see the possible probability manipulation of the watermark. 
    \item 1-gram can also be easily extended to c-gram by using a longer separator. So, the second assumption is the important one.
    \item  If the model without watermark has consistent (generation probability) behavior over different seprators and random words when doing such prompts, then we are still hopeful to figure out the distribution change to finish such a test (if the unwatermarked distribution is not very bad, intuitively speaking). 
\end{enumerate}

\subsection{Varun's thoughts}

\begin{enumerate}
\itemsep0em
\item We are assuming that the generation sequence is high entropy.
\item Generating token $t_i$ requires knowledge of tokens $\{t_{-i}\}$ (i.e., all tokens preceding it).
\item For a given token $t_i$ that is generated, with access to a proxy model (that is not watermarked), we know an ordered set of tokens $T_i$ from which it was chosen as the best token.
\item Since $t_i$ was generated, and verification relies on the generations containing a large number of ``green-list tokens'', we can assume that $t_i$ is a green-list token (w.h.p). % w.h.p.= with high probability
\item This means that $\hat{T}_i = T_i / \{t_i\}$ contains (marginally) more red-list tokens than green-list tokens (assuming $\gamma=0.5$).
\end{enumerate}

\noindent{\bf Attacker's goal:} As an attacker, we have knowledge of the ordered list $\hat{T}_i$, but do not know the colors of each token in this list. Let us assume that $\hat{T}_i$ contains the top 10 tokens (ordered by their score)\footnote{I know we are overloading notation here}. For small values of $\delta$, and high entropy sequences, the expectation is that $\hat{T}_i$ contains roughly an equal number of red and green tokens (\textcolor{red}{VC: Qilong, verify?}*
\textcolor{blue}{Qilong: Kind of confused here. Are we assuming that $t_i$ is a green-list token (w.h.p)?} \textcolor{red}{VC:yes}
). The task now is to reliably sample from this list a red-list token.

\textcolor{blue}{Qilong:
Assume we use top $k$, $k<<|\mathcal{V}|$. Then for unwatermarked proxy, color and $T_i$ are independent. The number of green tokens in $\hat{T}_i$ is about $N_g~B(k,0.5)-1$, the expectation is $k/2-1$, while the expectation for the number of red tokens is $k/2$. Note that this does not involve $\delta$.
}
\subsection{Random Replacement}
Let \( p = \frac{\|s\|_G}{T} \). Assume each token is green with probability \( p \) in watermarked text.
If we randomly replace \( s^{(t)} \), then the color of \( s^{(t)} \) and \( s^{(t+1)} \) may change. The expectation of green tokens for these two before replacement is \( 2p \), and after is \( 2\gamma \). If we do \( \frac{kT}{2} \) replacements (non-adjacent) in a string of \( T \) tokens, the expected number of green tokens becomes 
\[ \|s\|_G - \gamma T - 2(p-\gamma)\frac{kT}{2} = (1-k)(p-\gamma) T. \]
We need to replace every two tokens (e.g., 2nd, 4th, 6th, ...).

Conclusion: Approximately \( \frac{T}{2} \) replacements are necessary to change all tokens' color. Random replacement can only ``dilute."

\subsection{Our Testing}
For a pair of tokens \( (s^0s^1, s^0s^2) \) (where \( s^0 \) is for hashing), there are three possibilities:
\begin{enumerate}
    \item GR - green and red
    \item RG - red and green
    \item S - of the same color
\end{enumerate}
Our testing on \( (s^{(t-1)}s^{(t)}, s^{(t-1)}s^c) \) %and \( (s^{(t)}s^{(t+1)}, s^{c}s^{(t+1)}) \), 
where \( s^c \) is the candidate, shows that for each test (assuming independence), \( P(GR) = p(1-\gamma) \), \( P(RG) = (1-p)\gamma \), and \( P(S) = p\gamma + (1-p)(1-\gamma) \).

We will check the nominator of $\hat z$, which is $  \|s'\|_G - \gamma T $ after attack for each scheme. 

The following are commented out because: testing the color for \( (s^{(t)}s^{(t+1)}, s^{c}s^{(t+1)}) \) cannot be done directly (need to introduce additional reference).
\subsection{Scheme 5}
Instead of alternate replacement, we replace every token but only test \( (s^{(t-1)}s^{(t)}, s^{(t-1)}s^c) \). Also, note that the testing can be extended to multiple token pairs to be tested. Note that, if zero-temperature, multiple green tokens can have the same probability, leading to possible numerical issues. This may be mitigated if the temperature is low but non-zero.

\begin{enumerate}
    \item generate $m$ candidate tokens (using some model)
    \item similarity check (using another model) which gives $m'$ complaint candidates 
    \item do $m'+1$-test on $m'$ candidates and the original OR do at most $m'$ binary test as before until find a good candidate 
\end{enumerate}

\subsection{Scheme 6 - Close to Experiments but Token Level}
We start from the second token. Then we generate $m$ replacement candidates $(s^{c_1},\ldots,s^{c_m})$ and then do the test until the test result is GR or RG, or all candidates are used. We replace only when we get GR, then 
\begin{enumerate}
    \item advance by 2 if successful,
    \item advance by 1 otherwise.
\end{enumerate} 
This process is continued until we reach the end.

\subsubsection{Expected Green Ratio}
%Have not figured out how to compute the expectation of the number of green tokens after replacement. Yet this is stronger than Scheme 1 without additional computation (for each replacing attempt).
Assume our test is accurate. To figure out the estimated expected ratio $x$ of green tokens after the replacements, we need some mathematics. Assume all tokens can be replaced using the previous method (start at the first for simplicity, neglecting corner cases). Assume the color is independent of the candidates.

Let the expected number of green tokens after the attack (for $T$ tokens) be $e_T$. Let $p_s$ be the probability of successful replacement for each token (assume uniformity for simplicity). Let $e_2'$ be the expected number of green tokens for the replaced token and the token following it (2 tokens). Let $e_1'$ be the expectation of the number of green tokens for a token that is not replaced. Then we have:
\begin{equation}
e_T = p_s(e_{T-2} + e_2') + (1-p_s)(e_{T-1} + e_1')
\end{equation}
Let the expected ratio of green tokens be $x_T = e_T/T$. Let $x = \lim_{T \to \infty} \frac{e_T}{T}$. We have
\begin{multline}
T \cdot x_T = p_s(x_{T-2} \cdot (T-2) + e_2') \\
+ (1-p_s)(x_{T-1} \cdot (T-1) + e_1')
\end{multline}
$$
\text{Let } T \to \infty, \text{ then}
$$
\begin{multline}
T \cdot x = p_s(x \cdot (T-2) + e_2') \\
+ (1-p_s)(x \cdot (T-1) + e_1')
\end{multline}
\begin{equation}
x = \frac{p_s e_2' + (1-p_s)e_1'}{1 + p_s}
\end{equation}
For this particular scheme, we have
\begin{align*}
p_s &= p(1-p\gamma^m), \\
e_2' &= \gamma, \\
e_1' &= P(\text{token being green} | \text{attempt fails}) \\
&= P(\text{attempt fails} | \text{token being green})\\
&\cdot P(\text{token being green}) / P(\text{attempt fails}) \\
&= \frac{\gamma^m \cdot p}{1-p_s}.
\end{align*}
Plug in $x$:
\begin{equation}
x - \gamma = -\frac{\gamma(1-\gamma^m \cdot p)}{1+p(1-\gamma^m)} < 0
\end{equation}
So that we have enough replacements.
When $m \to \infty$, $x - \gamma \to -\frac{\gamma}{1+p}$.
\subsubsection{Success probablity}
% Introduction to the concept and definitions of variables
%The budget used for replacements, denoted as \( p_s \), is defined as the number of replacements over \( T \). The formula is given by:
For the success probability for each attempt with $k$ candidates
\begin{equation}
    p_s = p(1-p\gamma^m)
\end{equation}

\subsubsection{Expectation of Green Token Reduction}
The expectation of green token reduction per replacement is given by the following equation. This represents the average reduction in green tokens for each replacement event:
\begin{equation}
    1 + p - \gamma
\end{equation}

\subsubsection{LLM Call Expectations}
Let the expectation of LLM calls be \( n_T \). Let the expected ratio of LLM calls be \( y_T = \frac{n_T}{T} \).
As \( T \) approaches infinity, the expected number of LLM calls per attempt can be calculated. This is crucial for understanding the long-term behavior:
\begin{equation}
    \frac{\text{\# LLM calls}}{T} \to \frac{p\gamma + (1-p)(1-\gamma)}{(1+p)\gamma(1-\gamma)}
\end{equation}
For example, with \( p=0.5 \) and \( \gamma=0.25 \), this value approximates \( \frac{16}{9} \).

\subsubsection{LLM calls derivation}

\begin{align}
n_T &= \sum_{i=1}^{m} P(\text{success at the } i\text{-th time}) (n_{T-2} + i) \nonumber \\
    &\quad + (1 - p_s)(n_{T-1} + n_1')
\end{align}
Let \( y = \lim_{T \to \infty} \frac{e_T}{T} \). Let \( T \to \infty \), \( N_1' \) denotes the number of calls when there is no success with expectation \( n_1' \)
\begin{align}
Ty &= \sum_{i=1}^{m} P(\text{success at the } i\text{-th time})((T-2)y + i) \nonumber \\
   &\quad + (1-p_s)((T-1)y + n_1')
\end{align}


\[
y = \frac{\sum_{i=1}^{m} i P(\text{success at the } i\text{-th time}) + (1-p_s)n_1'}{1 + p_s}
\]
From this, we can get \( y \) for any \( m \), but the math is cumbersome. For simpler math, let \( m \to \infty \)
Then \( p_s = p \), \( N_1' \) is a geometric distribution with mean \( n_1' = \frac{1}{\gamma} \), 
\[
P(\text{success at the } i\text{-th time}) = p \gamma^{i-1} (1-\gamma)
\]
so
\[
\sum_{i=1}^{\infty} i P(\text{success at the } i\text{-th time}) = \frac{p}{1-\gamma}
\]
Plug in
\[
y = \frac{p \gamma + (1-p)(1-\gamma)}{(1+p) \gamma (1-\gamma)}
\]

\subsection{Discussion}

There is a trade-off between computation cost and effectiveness across the number of \( (s^{(t-1)}s^{(t)}, s^{(t-1)}s^c) \) candidates as expected.

\subsection{Extending scheme 6 to $c>1$}
We keep using scheme 6, then do the math for $c>1$. (Doable but the mathematics looks tricky after trails - leave for later).





==> notes/entropy.tex <==
\section{Entropy bounds}

\noindent{\bf Setting:}

\begin{enumerate}
\item Vocabulary size $|\mathcal{V}| \geq 4$. 
\item Shannon Entropy function with base $e$ be denoted as $H$. 
\item Spike entropy for constant parameter $z$ is defined as follows: $S(p, z) = \sum_k \frac{p_k}{1 + z p_k}$
\item $H(n):=H(1/n, ..., 1/n)$ 
\item $H(p):=H(p,1-p)$ (in the binary setting)
\item Let $l_i$ denote the $i^{th}$ largest logit score for $t^{th}$ tokens.
\item \begin{align*}
&\text{Let logit scores be}\\
&l_1 \geq  l_2 \geq, \ldots, l_{|\mathcal{V}|} \\
&\text{corresponding probabilities}\\
& p_1 \geq p_2 \geq \ldots \geq p_{|\mathcal{V}|} \\
\end{align*}
\item  $\alpha=e^\delta$
\end{enumerate}



\subsection{Case 1: $l_1 - l_2 \leq \delta$}
In this case, the entropy can be lower-bounded. It is straight-forward to verify both Shannon and Spike entropy are (strictly) concave. We can formalize the optimization problem as follows:

\begin{equation}
\begin{aligned}
& \underset{x}{\text{minimize}}
& & H(p_1,...,p_{|\mathcal{V}|}) \\
& \text{subject to}
& & \sum_{i=1}^{|\mathcal{V}|}{p_i}-1=0, \\
&&& p_i \geq p_{i+1}, \quad i=1,2,...,|\mathcal{V}|-1\\
&&& p_{|\mathcal{V}|} \geq 0\\
&&& p_1-\alpha p_2\leq 0, \quad
\end{aligned}
\end{equation}

We can see that all constraints are linear, and the set (for $p$) is convex (as all constraints are linear) and compact (subset of probability simplex).

The analogue minimum principle to the Bauer maximum principle is as follows:

Any function that is concave and continuous, and defined on a set that is convex and compact, attains its minimum at some extreme point of that set.

So we can reduce the problem to the extreme points. It is not hard to see that all extreme points are as follows:
\[
p_i =
\begin{cases}
\frac{\alpha}{\alpha+M-1} & \text{if } i=1, \\
\frac{1}{\alpha+M-1}  & \text{if } i=2,...,M, \\
0  & \text{if } i\geq M+1, \\
\end{cases}
\]
and
\[
p_i =
\begin{cases}
\frac{1}{M} & \text{if } i=1,...M \\
0  & \text{if } i\geq M+1, \\
\end{cases}
\]

(For derivation, note that $p_1 = p_2$ and $p_1=\alpha p_2$ cannot hold at the same time, enumeration can be greatly simplified.)
Plug in these two kinds of extreme cases, we can see that they are functions w.r.t. $M$. Using single variable calculus, we can show that the minimum are (for both the Shannon Entropy and Spike Entropy)
$$\ln(\alpha+1)-\frac{\alpha}{\alpha+1}\ln(\alpha) \quad for\ Shannon\ Entropy$$
$$\frac{\alpha}{\alpha + 1 + z \alpha} + \frac{1}{1 + \alpha + z} \quad for\ Spike\ Entropy$$
which are reached $\iff$
$$(p_1,...,p_{|\mathcal{V}|})=(\frac{\alpha}{\alpha+1}, \frac{1}{\alpha+1},0...,0)$$


\begin{comment}

\begin{align*}
&H(p_1, \ldots, p_k) \geq  H\left(\frac{p_1}{p_1+p_2}, \frac{p_2}{p_1+p_2}\right) = H \left( \frac{e^{l_1}}{e^{l_1} + e^{l_2}} \right) \\
&= H \left( \frac{1}{e^{l_2 - l_1} + 1} \right)\\
&\geq H \left( \frac{1}{1+e^\delta} \right) \\
&=\ln(e^\delta+1)-\frac{\delta e^{\delta}}{e^\delta+1}\\
&\text{``='' holds $\iff$ } l_1 - l_2 = \delta, \quad l_3 = \ldots = l_k = -\infty \\
\end{align*}
\end{comment}
\subsection{Case 2: $l_1 - l_2 \geq \delta $}
\subsubsection{A more general method}
%Using the fact that both Shannon and Spike entropy are concave, we can use Jensen's inequality:
Note that for either Entropy, the term for $p_i=p_i\ln(1/p_i)$ and $p_i=\frac{p_i}{1 + z \cdot p_i}$ are strictly concave. Using Jensen's inequlity, we have:
\begin{align*}
H(p_1,...,p_{|\mathcal{V}|}) &= p_1\ln\left(\frac{1}{p_1}\right) + \sum_{i=2}^{|\mathcal{V}|}p_i\ln\left(\frac{1}{p_i}\right) \\
                &\leq p_1\ln\left(\frac{1}{p_1}\right) \\ 
                &+ (|\mathcal{V}|-1)\left(\frac{1-p_1}{|\mathcal{V}|-1}\right)\ln\left(\frac{|\mathcal{V}|-1}{1-p_1}\right) \quad \\
                &for\ Shannon\ Entropy
\end{align*}
\begin{align*}
H(p_1,...,p_{|\mathcal{V}|}) &= \frac{p_1}{1+zp_1}+ \sum_{i=2}^{|\mathcal{V}|}\frac{p_i}{1+zp_i}\\
                &\leq \frac{p_1}{1+zp_1} + (|\mathcal{V}|-1)\frac{\frac{1-p_1}{|\mathcal{V}|-1}}{1+z\frac{1-p_1}{|\mathcal{V}|-1}}\quad \\
                & for\ Spike\ Entropy
\end{align*}
Take the right-hand side as functions of $p_1$, using single-variable calculus techniques, we can see both case are minimized at $p_1=\frac{\alpha}{|\mathcal{V}|-1+\alpha}$. As the $=$ for Jensen's inequlity holds $\iff p_2=...=p_{|\mathcal{V}|}$ So $p_i=\frac{1}{|\mathcal{V}|-1+\alpha}, \quad i=2,3,...,|\mathcal{V}|$, we can conclude that the maixmum are:
$$
\ln(\alpha+|\mathcal{V}|-1)-\frac{\alpha}{\alpha+|\mathcal{V}|-1}\ln(\alpha)\\
\quad
$$
for Shannon Entropy
$$
\frac{\alpha}{\alpha + |\mathcal{V}| - 1 + z\alpha} + \frac{(|\mathcal{V}| - 1)(\alpha + |\mathcal{V}| - 1)}{\alpha + |\mathcal{V}| - 1 + z}\\
$$
for Spike Entropy

which are reached $\iff$
\begin{align*}
    &(p_1,...,p_{|\mathcal{V}|})=\\
&(\frac{\alpha}{\alpha+|\mathcal{V}|-1}, \frac{1}{\alpha+|\mathcal{V}|-1},...,\frac{1}{\alpha+|\mathcal{V}|-1})
\end{align*}

\subsubsection{Previous method}
This methods is only for Shannon Entropy
\begin{align*}
& \text{Let $c=p_1+p_2$} \\ 
&H(p_1, \ldots, p_k) = H(c)+cH \left( \frac{p_1}{p_1 + p_2} \right) \\
&+ (1 - c) H \left( \frac{p_3}{1 - c}, \ldots, \frac{p_{|\mathcal{V}|}}{1 - c} \right) \\
& \leq H(c) + c H \left( \frac{1}{1+e^\delta} \right) + (1 - c) H(|\mathcal{V}| - 2) \\
&= H(|\mathcal{V}|-2)+(H \left( \frac{1}{1+e^\delta} \right)-H(|\mathcal{V}|-2))c+H(c)\\
&:=f(c)\\
%&H \leq \left( H \left( e^\delta \right) - H(|\mathcal{V}|-2) \right) \left( 1 - \frac{|\mathcal{V}|-2}{e^\delta + |\mathcal{V}| - 1} \right) \\
%&= \left( 1 - \frac{|\mathcal{V}|-2}{e^\delta + |\mathcal{V}| - 1} \right) H \left( e^\delta \right) + \frac{|\mathcal{V}|-2}{e^\delta + |\mathcal{V}| - 1} H(|\mathcal{V}|-2)
\end{align*}
\begin{align*}
    f'(c)&=-\ln(c/(1-c))+H \left( \frac{1}{1+e^\delta} \right)-\ln(|\mathcal{V}|-2)\\
    f''(c)&=-\frac{1}{c(1-c)}<0
\end{align*}
So $f'(c)$ monotonously decreases. Also,
\begin{align*}
    c=&p_1+p_2\\ 
    &= \frac{exp(l_1)+exp(l_2)}{exp(l_1)+...+exp(l_{|\mathcal{V}|})}\\
    &\geq \frac{exp(l_1)+exp(l_2)}{exp(l_1)+(|\mathcal{V}|-1)exp(l_2)}\\
    &= \frac{exp(l_1-l_2)+1}{exp(l_1-l_2)+(|\mathcal{V}|-1)}\\
    &\geq \frac{e^{\delta}+1}{e^{\delta}+(|\mathcal{V}|-1)}
\end{align*}
So
\begin{align*}
    f'(c)&\leq f(\frac{e^{\delta}+1}{e^{\delta}+(|\mathcal{V}|-1)})\\
         &=-\ln\frac{e^{\delta}+1}{|\mathcal{V}|-2}\\
         &+\frac{1}{1+e^\delta}\ln(1+e^{\delta})\\
         &+\frac{e^{\delta}}{1+e^\delta}ln(\frac{1+e^\delta}{e^{\delta}})
         -\ln(|\mathcal{V}|-2)\\
         &=-\frac{\delta e^{\delta}}{1+e^\delta} < 0
\end{align*}
Consequently, $f(c)$ monotonously decreases. We have:
\begin{align*}
    H &\leq f(\frac{e^{\delta}+1}{e^{\delta}+(|\mathcal{V}|-1)})\\
        &=\ln(e^\delta+|\mathcal{V}|-1)-\frac{\delta e^{\delta}}{e^\delta+|\mathcal{V}|-1}\\
&\text{``='' holds $\iff$ } l_1 - l_2 = \delta, \quad l_2=l_3 = \ldots = l_{|\mathcal{V}|} 
\end{align*}
\subsection{Discussion}
\subsubsection{Remarks}
\begin{enumerate}
    \item Note that the above entropy lower-bound only involves $\delta$ and the upper-bound only involves $\delta$ and $|\mathcal{V}|$.
    \item When $|\mathcal{V}|=2$, the two bounds degenerate to the same value.
\end{enumerate}
\subsubsection{Extension to other entropy definitions}

The above bounds can be extended to other definitions of entropy.

If the entropy is concave, we can reduce to extreme points for minimum as the set is convex and compact.

If the entropy is concave and is in the form of $\sum f(p_i)$, then we may use similar techniques to find the maximum using Jensen's inequality. The form of $\sum f(p_i)$ can be relaxed to symmetric (which should hold for all entropy definitions).

Let \( S_{n-1} \) be the symmetric group of all permutations of \( n-1 \) elements, where \( n = |\mathcal{V}| \). Then use the Jensen's inequality over the sum over all permutations \( \sigma \) of \( S_{n-1} \) applied to the function \( H \), which is symmetric in its last \( n-1 \) arguments:

\begin{align*}
&(n-1)! \cdot H(p_1, p_2, \ldots, p_n)\\
&= \sum_{\sigma \in S_{n-1}} H(p_1, p_{\sigma(2)}, \ldots, p_{\sigma(n)}) \\
&\leq (n-1)! \cdot H\left(p_1, \frac{1-p_1}{n-1}, \ldots, \frac{1-p_1}{n-1}\right)
\end{align*}

where the division by \( n-1 \) distributes the remaining quantity \( 1-p_1 \) equally among the \( n-1 \) arguments.


%The problem is that the implication of such results are not very clear. 
\subsubsection{Implication}
For simplicity, we assume temperature to be 0 and we are using Shannon entropy.

1. We can confirm that when the entropy is less than the lower-bound (for typical value $\delta=2$, this is 0.527 bits), the watermark will not make a difference. This implies that if we can let the model to always generate low-entropy tezt, watermark can be evaded. 

2. If\ it is impossible for the watermark to change the output, the entropy is upper-bounded but it is very close to the unconstrained upperbound. That is because for typical value $\delta=2$, $|\mathcal{V}|=50527$ for GPT2-xl while similar for other models, this is 15.6245 bits, while the upper-bound without constraints is 15.6248 bits. 
%Bounding entropy also looks like a well-defined optimization problem, so it might also be solved using more general techniques.
%What we used for $H$:
%1. Non-negative
%2. Reduction on condition
%3. $H(p)$ monotonously increasing from on $[0,1/2]$.
%4. Additivity.
%5. 

% Marked as TODO
\textcolor{red}{VC: What is missing here is how do you connect this gap in logit scores to "success" in their verification algorithm? for that, it would be helpful to (a) re-write the above using the same notation as they have used in their paper, and (b) also describe their 
verification mechanism? it is a one-sided hypothesis test involving what?}

%\textcolor{blue}{Qilong: marked as TODO.}
\textcolor{blue}{Qilong: The quantity they are testing:
$$\hat{z} = \frac{\|s\|_G - \gamma T}{\sqrt{T \gamma (1 - \gamma)}}$$. $T$ is the number of tokens, $\|s\|_G$ is the number of green tokens in these $T$ tokens. The threshold of $z$ is set to 4. They are using spike entropy instead of Shannon entropy ($z=4$) as defined above.
%Trying to extend to this entropy from Shannon entropy.
}



==> old/4_contributions.tex <==
\newpage
\section{Main Technical Contributions}
% need to be made more formal
In this section, we will first show some properties of the watermarking scheme on scaling to length, then why existing color-agnostic attack methods will fail for sufficiently long watermarked text, then we focus on substitution-based attack and include the color-agnostic baseline. Based on this, we present our attack and do a similar analysis showing its scalability and also the required LLM calls.
%We will first show why existing color-agnostic attack methods will fail for sufficiently long watermarked text, then the ideal color-aware substitution case, then our solution and corresponding analysis
%\varun{write a small blurb on what the main point of this section is} \ql{updated. if it is too long, we can move some to the appendix for which the only difference is some constants in the bound}

\subsection{Assumptions and Definitions}

\noindent{\bf Assumption 1:} We consider the left hash. Self hash is similar. Left (self) hash means the green list for the current token is hashed from $c$ tokens counting backwards from the previous (current) token. %\varun{more details on what left hash is} \ql{updated}

\noindent{\bf Assumption 2:} Assume each token is green with constant probability $p$ in watermarked text, i.i.d, s.t. $ \gamma < p < 1$. The number of $c-$grams is then $T-c$. %Assume independent from $T$.

\noindent{\bf Definition 1.} \underline{$c+1$-gram}: \varun{recall that at each step of generation, the final $c+1$ input tokens that are fed as input to the generative model are used for color determination before generation. we term this sequence a $c+1$ gram.} The minimum unit used for one color testing, including the token whose color is to be checked and the $c$ tokens before it. When we say the color of a $c+1$-gram, we mean the color of the last token, equivalently the color result when this $c+1$-gram is sent to the detector. 

\noindent{\bf Definition 2.} \underline{Effective $T$ ($T_e$):} the number of $c+1$-grams for color testing i.e., $T_e=T-c$

\noindent{\bf Definition 3.} \underline{Detection threshold ($z_{th}$)}: The threshold used in detection. Detector output "watermarked" $\iff z > z_{th}$. 

\noindent{\bf Definition 4.} \underline{Critical length ($T_c$)}: This is the value of $T_e$ such that $\mathbb{E}[z]=z_{th}$. This is roughly how many effective tokens are needed for successful detection and may or may not exist.


\subsection{Theorem}

\varun{the theorem should have some written statement as well i.e., "The probability of being labeled as unwatermarked converges to 0 exponentially w.r.t. $T_e$.
" seems like a good statement. then everything else that follows seems like the proof?}

\ql{Mostly. Watermark strength $\propto \sqrt{T_e}$ and probability of the opposite direction -> 0 exponentially. The following are listing results under strong to weak assumptions.}

% \input{contents/theorem}

\subsection{Why Existing Methods do not Work for Long Text}
\subsubsection{Unattacked Text}
Apply the theorem (\ref{iidth}, $q=p$, i.i.d. case) we can see that the false positive rate converges to $0$ exponentially w.r.t. $T_e$.
\subsubsection{Attack 1}
There are attacks like designing prompts to guide the watermarked model to generate low-entropy texts to evade detection, where it is harder to incorporate watermarks into more deterministic texts. However, we will see that it may only dilute the watermark.

Assume the attacker can reduce $p$ to $p'$, but $p'>\gamma$, i.e., the $c+1$-grams are $i.i.d.$ green with probability $p'$. Then the above still holds except we use $p'$ instead of $p$.

\noindent{\bf Conclusion}
This attack would fail for sufficiently long watermarked text because it can only dilute the watermark.

\subsubsection{Attack 2}
In this attack, the attacker is using color-agnostic post-processing methods, i.e., color-agnostic post-processing is applied to watermarked text to evade detection. Existing paraphrasing-based methods \citep{lu2023large, krishna2023paraphrasing} fall into this category. We will see these methods still can only dilute the watermark.
%We assume the post-processed text includes two parts of $c+1$-grams.
%$$0 < \mathbb{E}[z'] =\frac{p'-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T}\propto \sqrt{T}$$, and standard deviation is still a constant $$\sigma_z'=\sqrt{\frac{p'(1-p')}{\gamma(1-\gamma)}}$$. Then this method would fail for sufficiently large $T$. This corresponds to the result in \citet{kirchenbauer2023reliability}. 

\varun{need some explanation here on what you are doing, and what you hope to achieve}


\noindent{\bf Assumptions}
\begin{itemize}
    \item The post-processing is color-agnostic. We assume the new $c+1$-grams are green with i.i.d. probability $\gamma$, and the number of such new $c+1$-grams is $T_{n}$. We call them new $c+1$-grams.
    \item Postprocessing like paraphrasing is statistically likely to leak n-grams or even longer fragments of the original text \citep{kirchenbauer2023reliability}. We call them old $c+1$-grams. These old $c+1$-grams are green with i.i.d. probability $p$ from the previous assumption, and the number of such old $c+1$-grams is $T_{o}$. 
    \item The above two composes post-processed text's $c+1$-grams, implying $T_e=T_o+T_n$ when detecting the watermarking from the attacked text.
    \item $c+1$-gram leaking ratio $r_o=\frac{T_o}{T_o+T_n}$, is a positive constant independent from $T_e$.
    \item The color for different $c+1$-grams are independent.
\end{itemize}

%$$\sigma_{z''}=\sqrt{\frac{\gamma(1-\gamma)(1-r_o)+\Pr(1-p)r_o}{\gamma(1-\gamma)}}$$ is a constant.
\noindent{\bf Definition}
\begin{itemize}
    \item $\|T\|_G^o$: the number of green old $c+1$-grams as a random variable
    \item $\|T\|_G^n$: the number of green new $c+1$-grams as a random variable
\end{itemize}
So $\|T\|_G^o\sim B(T_o,p)$, $\|T\|_G^n\sim B(T_n,\gamma)$, $\|T\|_G=\|T\|_G^o+\|T\|_G^n $.

Apply the independent case of the theorem (\ref{indth}), the probability of evading detection exponentially converges to $0$ w.r.t. $T_e$.

\noindent{\bf Remark 1}
In paraphrasing, we can safely assume when the watermarked text being paraphrased becomes longer, the paraphrased text becomes longer accordingly.

\noindent{\bf Conclusion}
This attack would fail for long enough generated text when a non-zero ratio of $c+1$-grams is preserved. % need to be more precise here
%More specifically: 
%\ql{add argument computing standard deviation here}

\noindent{\bf Remark 2}
Even if attack 1 and attack 2 are combined, i.e., the attacker can weaken the watermark and do color-agnostic post-processing, then it would still fail for sufficiently long text. To see this, just let $p=p'>\gamma$ in the above derivation.

\subsection{\bf General Substitution}
%\ql{problem: this extension does not hold for our attack, and only applied once besides the removed hypothetical color-aware attack, making it not so useful}

\noindent{\bf Assumption 1}
For simplicity, we assume $c=1$. Then $c+1$-grams are $2$-grams, $T_e=T-1$. Larger $c$ are essentially similar. This assumption is for all remaining parts of this section.

% our method is far from this, may remove later
We have shown the weakness of color-agnostic methods. Let $0<r_n\leq 1$ be constant independent from $T_e$. Assume we have made $\frac{r_n T_e}{2}$ non-adjacent substitutions. To maximize the number of new $2$-grams given fixed number of substitutions, as one substitution changes up to two $2$-grams, we assume exactly two for simplicity. 

\noindent{\bf Grouping}
We divide $r_n T_e$ new $2$-grams to $\frac{r_n T_e}{2}$ 2-group, where $2$-grams are in the same group $\iff$ they are new because of the same substitution. The old $2$-grams are grouped in one $2$-gram one-group manner. \label{GeneralGrouping}

\noindent{\bf Assumption 2}
\begin{itemize}
    \item The number of green $2$-grams in each new $2$-gram group (two $2$-grams) are random variables with expectation $2p_n$.
    \item The number of green $2$-grams in each old $2$-gram group (one $2$-gram) are random variables with expectation $p_o$.
    \item The number of green $2$-grams of different groups are independent.
\end{itemize}

Average green probability $\overline{p}=r_n p_n+(1-r_n)p_o$. Even if the theorem cannot be directly applied, similar results can be derived. When $\overline{p}>\gamma$, the probability to evade watermarking exponentially converges to $0$ w.r.t. $T_e$; when $\overline{p}<\gamma$, the probability of failing to evade watermarking exponentially converges to $0$ w.r.t. $T_e$. More details are in the appendix. 

\noindent{\bf Conclusion} If substitution attacks can scale to arbitrarily long text depends on if the average green probability is at most $\gamma$.

\subsubsection{\bf Color-agnostic Substitution Baseline}
From above, we do color-agnostic substitutions, so that we assume $p_n=\gamma$, $p_o=p$. Then $\overline{p}=r_n \gamma +(1-r_n)p \geq \gamma$. Consequently, unless $r_n=1$, the probability of evading watermarking exponentially converges to $0$ w.r.t. $T_e$. This implies almost at least half of the substitutions are required.

\ql{removed ideal color-aware substitution as it is not that ideal and important}
\subsection{Our Approach: Self Color Testing (SCT)} 

\noindent{\bf Key Insight}
The key to a successful attack against watermarked LLM is to have color information. This is not easy, but we can do it by prompting the model to generate a random string and infer color information from the frequency.

We make the following adaptation for prompting:  
\begin{itemize}
\item We work on the word level to avoid some encoding issues and incomplete word biases.
\end{itemize}

\begin{algorithm}
\SetAlgoLined % This sets line numbering on, but you can remove it if you don't want line numbers
\textbf{Input:} $w_b$, $w_b'$, $w_b^c=w_{b-c}\ldots w_{b-1}$\;
\textbf{Output:} Test result in $\{GR,RG,S\}$. $GR$ ($RG$) means $w_b$ is green (red) while $w_b'$ is red (green)\;

$p=\text{prompt}(w_b, w_b', w_b^c)$\;
$text=\text{LLM}(p)$\;
$c_b, c_b' = \text{count}(text, w_b^cw_b), \text{count}(text, w_b^cw_b')$\;
$p_t=\chi^2\text{-test}(c_b, c_b')$\;
  \If{$p_t \geq p_{th}$}{
    \Return $S$\;
    }
    \uElseIf{$c_b>c_b'$}{
    \Return $GR$\;
    }
    \Else{
    \Return $RG$\;
    }
\caption{Self Color Testing}
\end{algorithm}

We make further assumptions for the ease of understanding:


\noindent{\bf Assumptions}
\begin{enumerate}
    \item Temperature $t=0$, meaning deterministic generation from probabilities.
    \item The LLM's random generation follows the prompt's instruction.
\end{enumerate}

And our example prompt for color testing is as follows $(w_b=includes, w_b'=contains, w_b^c=kernel)$:
Choose two phrases ( kernel includes, kernel contains ), and generate a long uniformly random string of those words separated by ";". Previous phrases should have no influence on future phrases: kernel includes; kernel contains; kernel includes; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains; kernel includes; kernel contains; kernel contains;

Here the word "includes" is the word being substituted, "contains" is the candidate word. Then we check the frequency of the response for this prompt.

Assume the token before "includes" and "contains" are the same in the encoded "kernel includes" and "kernel contains". 
%\begin{itemize}
%    \item Do a $\chi^2$ test.
%    \item If p-value $\geq$ threshold, then we conclude they are both green or both red.
%    \item If p-value < threshold, then the lower frequency one is red and the higher one is green.
%\end{itemize}
Then as the model is deterministic, and the model follows the prompt's probability, the model will always generate the green one if $w_b$ and $w_b'$ are of different colors, so SCT has a perfect recall on $GR$ and $RG$. For $S$ there can be border cases but in realistic applications, $t>0$ so they will have the same probability of appearing. 

\noindent{\bf SCTS}
The idea is to use color-testing to test different candidates to try to ensure that the token is substituted from green to red.

%\noindent{\bf Algorithm}

\begin{algorithm}
\SetAlgoLined % This sets line numbering on, but you can remove it if you don't want line numbers
\textbf{Input:} $w$, \\
\textbf{Output:} $w'$\\
\textbf{Initialization:} $i=c$, $w'=w$\\
\While{$i \leq n$}{
    $w_{b1},\ldots,w_{bk} = \text{generate\_candidates}(w', i)$\\
    $success=\text{False}$\\
    \For{$j=1$ \KwTo $k$}{
        \If{$\text{SCT}(w_i, w_{bj}, w_{i-c}\ldots w_{i-1}) == \text{GR}$}{
            $w'=\text{Substitute}(w',i,w_{bj})$\\
            $success=\text{True}$\\
            break
        }
    }
    \eIf{success}{
        $i\gets i+2$\\ advance by 2 for economic substitution
    }{
        $i\gets i+1$\\
    }
}
\caption{SCTS Algorithm}
\end{algorithm}
\noindent{\bf Budget enforcement}
To enforce the budget, we add checking if the budget is reached after each replacement based on the previous SCTS.


\subsection{\bf SCTS analysis}
We make the following further assumptions:
\begin{itemize}
    \item One token per word for simplicity (or token-level attack)
    \item Candidate generation process is independent from the red and green list, i.e., every candidate is green with $i.i.d.$ probability $\gamma$.
\end{itemize}

\noindent{\bf Success Rate}
For each $2$-grams' substitution attempt, the success probability
$$
p_s=p(1-\gamma^k)
$$

\noindent{\bf Expected Green Ratio}
%Have not figured out how to compute the expectation of the number of green tokens after replacement. Yet this is stronger than Scheme 1 without additional computation (for each replacing attempt).
Let $q(T_e)$ be the average green probability.

When $k>1+\log_\gamma \frac{1-p}{p(1-\gamma)}$
\begin{align}
q(T_e)\leq \max \{\frac{\gamma}{2}, \frac{\gamma^k p}{1-p+\gamma^k p}\} < \gamma
\label{eq:qTeBound}
\end{align}
\begin{equation}
\lim_{T_e \to \infty} q(T_e) = \gamma - \frac{\gamma(1-p\gamma^{k-1})}{1+(1-\gamma^k)p} < \gamma
\label{eq:limit_expression}
\end{equation}

Using similar techniques as 4.4, we have
\begin{align}
    \Pr(z > z_{th}) < &\exp\Bigg(-(\gamma-q(T_e))^2\Bigg(\sqrt{T_e} \nonumber \\
    &\quad +\frac{\sqrt{\gamma(1-\gamma)}z_{th}}{\gamma-q(T_e)}\Bigg)^2\Bigg)
    \label{eq:ProbabilityBound}
\end{align}

 for $q(T_e)<\gamma$, which holds for large enough $k$ and/or $T_e$.
So that the probability of failing to evade the watermark converges to $0$ exponentially.
This means in expectation our method can reduce the average green probability to less than $\gamma$, and it is scalable to arbitrarily long text. More details are in the appendix.

\noindent{\bf LLM Call Expectations}

Let the number of LLM calls be \( N_{T_e} \). 
\begin{equation}
\begin{split}
&\mathbb{E} [N_{T_e}] \\
\leq& \max \Bigg\{ \frac{1}{2} \left( \frac{1}{\gamma} - \left( \frac{1}{1-(1 - \gamma)^k} - 1 \right)k \right), \\
&\qquad \frac{1-\gamma^k}{1-\gamma} \Bigg\}T_e \\
< &\max \left\{ \frac{1}{2\gamma}, \frac{1}{1-\gamma} \right\}T_e
\end{split}
\label{eq:LLMcallsbound}
\end{equation}


As \( T_e \to \infty \) and $k \to \infty $, the expected number of LLM calls per $c+1$-gram can be estimated. This is crucial for scalability.
\begin{equation}
    \lim_{T_e, k \to \infty} \frac{\mathbb{E}[N_{T_e}]}{T_e}  = \frac{p\gamma + (1-p)(1-\gamma)}{(1+p)\gamma(1-\gamma)}
    \label{eq:LLMcallslimit}
\end{equation}
For example, with \( p=0.5 \) and \( \gamma=0.25 \), this value is \( \frac{16}{9} \).

Also, $N_{T_e}$ will not deviate far from its expectation with high probability.
 \begin{equation}
    \Pr (|\frac{N_{T_e}-\mathbb{E}[N_{T_e}]}{T_e}| \geq t) \leq \frac{C}{T_et^2}
    \label{SCTSPrBound}
\end{equation}
For $t>0$ and constant
\begin{equation}
\begin{split}
&C\coloneqq
\\ & \max
\Bigg\{
\frac{1}{2} \left(\frac{1 - \gamma}{\gamma^2}-\frac{k^2 (1 - \gamma)^k}{(1 - (1 - \gamma)^k)^2}\right),\\
& \frac{\gamma}{(1-\gamma)^2} - \frac{\gamma^k ((2k-1)(1-\gamma) + \gamma^k)}{(1 - \gamma)^2}
\Bigg\}\\
<& \max \Bigg\{  \frac{1-\gamma}{2\gamma^2}, \quad \frac{\gamma}{(1-\gamma)^2}  \Bigg\}
\end{split}
\end{equation}

Consequently, our method is reasonably fast, with $O(1)$ w.r.t. $k$, and $O(T_e)$ w.r.t. $T_e$.
The proof is in the appendix. 

\varun{looks good till here}

%\ql{no bound here because didn't find a way to bound variance, and the color for each grouping does not seem independent}

==> old/theorem.tex <==
\noindent{\bf Case 1:  i.i.d. case.} Let $D(a||q)$ be KL-divergence with base $e$:
$$D(a||q)\coloneqq a \ln \frac{a}{q}+(1-a)\ln{\frac{1-a}{1-q}}$$
Assume the $c+1$-grams are green with i.i.d. probability $q$. Then:
$$\mathbb{E}[z] =\frac{q-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e}$$

\begin{enumerate}
\item[S1.] If $q > \gamma $, then $\mathbb{E}[z]  \propto \sqrt {T_e}$ and 
$T_c=\frac{\gamma(1-\gamma)z_{th}^2}{(q-\gamma)^2}$

For $T_e \geq T_c$,

\varun{by chernoff bound?}
\begin{equation}
\begin{split}
  &\Pr(z \leq z_{th}) \\
  \leq &\exp\left(-T_eD\left(\frac{\sqrt{\gamma(1-\gamma)} z_{th}}{\sqrt{T_e}}+\gamma || q \right)\right)
\end{split}
\label{eq:iid_bound_1}
\end{equation}
$\implies$ Probability of being labeled ``unwatermarked'' converges to 0 exponentially w.r.t. $T_e$.

\item[S2.] If $q=\gamma$, then $\mathbb{E}[z] = 0$, and $T_c$ does not exist. 

$$\lim_{T_e\to \infty} \Pr(z>z_{th}) = 1-\Phi(z_{th})$$.

$\implies$ Probability of being labeled as ``watermarked'' converges to a positive constant. Typical value $z_{th}=4$, $1-\Phi(z_{th})\approx 0.00003167$.

\item[S3.] If $q < \gamma$, then $\mathbb{E}[z]  \propto - \sqrt {T_e}$, and $T_c$ does not exist.
\begin{align*}
    &\Pr(z > z_{th})\\
\leq&\exp\left(-T_eD(\frac{\sqrt{\gamma(1-\gamma)} z_{th}}{\sqrt{T_e}}+\gamma || q)\right)
\end{align*}

%The probability of being labeled as watermarked converges to 0 exponentially w.r.t. $T_e$.
$\implies$ Probability of being labeled ``watermarked'' converges to 0 exponentially w.r.t. $T_e$.
\end{enumerate}

%\label{indth}
%The key i the average probability for the $c+1$-grams being green
\noindent{\bf Case 2: Independent case.} Assume the $c+1$-grams' colors are independent. Let the average probability of being green for $T_e$ $c+1$-grams be $q$. Then:

$$\mathbb{E}[z] =\frac{q-\gamma}{\sqrt{\gamma(1-\gamma)}}\sqrt{T_e}$$
\begin{enumerate}
\item[S1.] If $q > \gamma $, 
$\mathbb{E}[z]  \propto \sqrt {T_e}$ and  $T_c=\frac{\gamma(1-\gamma)z_{th}^2}{(q-\gamma)^2}$

Besides:
\begin{equation}
\begin{split}
&\Pr(z \leq z_{th}) \\
\leq &\exp \left(-2(q-\gamma)^2(\sqrt{T_e}-\sqrt{T_c})^2\right)
\end{split}
\label{eq:IndBound}
\end{equation}

$\implies$ Still, the probability of being labeled as unwatermarked converges to 0 exponentially w.r.t. $T_e$.

\item[S2.] If $q=\gamma$, $\mathbb{E}[z] = 0$ and $T_c$ does not exist.

\item[S3.] If $q < \gamma$, $\mathbb{E}[z]  \propto - \sqrt {T_e}$ and $T_c$ does not exist. 
Besides:
\begin{equation}
\begin{split}
        &\Pr(z > z_{th})\\
    \leq &\exp(-2(\gamma-q)^2(\sqrt{T_e}+\frac{\sqrt{\gamma(1-\gamma)}z_{th}}{\gamma-q})^2) 
\end{split}
\label{eq:IndBound2}
\end{equation}

$\implies$ Still, the probability of being labeled as watermarked converges to 0 exponentially w.r.t. $T_e$.
\end{enumerate}

